ARRAKIS: Atlas of Resonance Rings As Known In the S4G

Resonance rings are the consequence of secular evolution processes that redistribute material and angular momentum in discs. We produced a Catalogue and an Atlas of the rings detected in the Spitzer Survey of Stellar Structure in Galaxies (S4G) and to conduct a statistical study of the data in the Catalogue. We traced the contours of rings previously identified by Buta et al. (in preparation) and fitted them with ellipses. We found the orientation of bars by studying the galaxy ellipse fits from S4G's Pipeline 4. We used the galaxy orientation data obtained by S4G's Pipeline 4 to obtain intrinsic ellipticities and orientations of rings and the bars. ARRAKIS contains data on 724 ringed galaxies in the S4G. The frequency of resonance rings in the S4G is of 16+-1% and 35+-1% for outer and inner features, respectively. Outer rings are mostly found in Hubble stages -1<=T<=4. Inner rings are found in a distribution that covers the range -1<=T<=7. We confirm that outer rings have two preferred orientations, parallel and perpendicular to the bar. We confirm a tendency for inner rings to be oriented parallel to the bar, but we find that a significant fraction (~50%) of them have random orientations with respect to the bar. These misaligned inner rings are mostly found in late-type galaxies (T>=4). This may be due to spiral modes decoupled from the bar dominating the Fourier amplitude spectrum at the radius of the inner ring. We find that the fraction of barred galaxies hosting outer (inner) rings is ~1.7 times (~1.3 times) that in unbarred galaxies. The fact that rings are only mildly favoured by bars suggests that those in unbarred galaxies either formed due to weak departures from the axisymmetry of the galactic potential or that they are born because of bars that have been destroyed after the ring formation.

==> atlas.tex <==
\clearpage
\onecolumn
\section{Atlas}
The atlas contains two sets of galaxies. One for galaxies included in the S$^4$G sample and a second one for galaxies that appear in S$^4$G frames, but are not included in the original sample. The information in the atlas is organized as follows:
\begin{itemize}
\item Line~1: Galaxy ID
\item Line~2: Galaxy classification according to Buta et al.~(in preparation).
\item S$^4$G original galaxy image and P4 model-subtracted image (Salo et al.~in preparation). The red ellipses indicate the rings in the galaxy. The green ellipses are the result of an ellipse fit at the radius of the maximum bar ellipticity. The red crosses indicate the centre of the galaxy. The axis units are arcseconds. North is up and east is left.
\item Below this information we present a table showing the information on the projected and deprojected information on the rings, pseudorings, and bars of that galaxy as shown in the catalogue in Appendix~A.
\end{itemize}
\clearpage
\subsection{Atlas of galaxies in the S$^4$G sample that host rings}
\begin{longtable}{c c c c c c c | c c c c c c c}
\multicolumn{7}{c}{{\large{\bf ESO~13-16}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~26-1}}}\\
\multicolumn{7}{c}{SB(rs)cd }&
\multicolumn{7}{|c}{(R$_{2}^{\prime}$)SAB(s)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO013-016.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO026-001.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.78&0.66&161.7&1.01&0.78&92.5&
R$_{2}^{\prime}$&1.25&0.92&37.4&1.26&0.97&22.3\\
bar&0.30&0.08&166.0&0.30&0.12&0.5&
bar&0.23&0.07&66.9&0.24&0.08&49.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~54-21}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~119-16}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(s)d pec }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(s)dm: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO054-021.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO119-016.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&3.15&1.55&101.6&3.78&2.65&53.9&
R$^{\prime}$&2.24&0.56&30.3&2.33&1.50&22.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~202-41}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~234-49}}}\\
\multicolumn{7}{c}{SB(rs)m }&
\multicolumn{7}{|c}{SA(r)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO202-041.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO234-049.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.85&0.75&174.4&1.13&0.83&82.9&
r&0.24&0.12&170.7&0.25&0.12&92.2\\
bar&0.73&0.22&166.9&0.75&0.32&19.9&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf ESO~240-11}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~285-48}}}\\
\multicolumn{7}{c}{SA(rs:)b sp }&
\multicolumn{7}{|c}{SB(rs)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO240-011.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO285-048.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.05&0.11&127.8&1.06&0.70&5.0&
rs&0.64&0.30&80.7&0.70&0.64&99.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~355-26}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~358-25}}}\\
\multicolumn{7}{c}{SA(r)bc }&
\multicolumn{7}{|c}{SA(l,nr)0$^{+}$/SA0$_{\rm d}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO355-026.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO358-025.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.23&0.17&154.7&0.32&0.23&91.0&
nr&0.14&0.09&57.4&0.15&0.14&75.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~362-19}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~399-25}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)d }&
\multicolumn{7}{|c}{(RL)E(d)2 }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO362-019.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO399-025.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.82&0.39&3.9&1.87&1.23&19.0&
RL&3.08&1.16&153.0&3.09&1.62&171.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf ESO~402-26}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~402-30}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)S${\underline{\rm A}}$B(r,nl)ab }&
\multicolumn{7}{|c}{SA(rs)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO402-026.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO402-030.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.80&0.61&113.0&1.91&1.59&38.9&
rs&0.18&0.07&134.4&0.18&0.12&171.4\\
r&0.61&0.27&100.4&0.83&0.56&111.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~404-12}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~407-7}}}\\
\multicolumn{7}{c}{SAB(${\underline{\rm r}}$s)b }&
\multicolumn{7}{|c}{SA(rl)a: sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO404-012.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO407-007.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&0.49&0.17&131.1&0.50&0.19&15.1&
rl&0.49&0.07&168.7&0.49&0.34&4.8\\
${\underline{\rm r}}$s&0.41&0.40&145.6&0.47&0.41&86.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~407-14}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~418-8}}}\\
\multicolumn{7}{c}{SA(r)ab }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(s)dm: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO407-014.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO418-008.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.41&0.16&40.3&0.41&0.30&0.6&
R$^{\prime}$&0.80&0.50&151.7&0.86&0.68&42.7\\
&&&&&&&
bar&0.13&0.04&9.0&0.17&0.04&63.8\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf ESO~420-9}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~422-5}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(rs)c }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$:)dm: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO420-009.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO422-005.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.40&0.36&76.9&0.50&0.38&81.2&
r${\underline{\rm s}}$&0.47&0.40&51.0&0.58&0.44&74.9\\
bar&0.12&0.06&39.8&0.12&0.08&13.0&
bar&0.25&0.13&79.5&0.32&0.14&69.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~422-41}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~440-4}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(l)c: }&
\multicolumn{7}{|c}{SAB(rl)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO422-041.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO440-004.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.26&1.87&91.1&2.39&2.15&55.8&
rl&0.98&0.75&82.4&1.80&0.98&87.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~440-11}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~443-69}}}\\
\multicolumn{7}{c}{SB(rs)cd }&
\multicolumn{7}{|c}{SB(rs)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO440-011.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO443-069.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.58&0.44&15.9&0.59&0.48&154.5&
rs&0.67&0.59&172.9&0.73&0.61&67.1\\
bar&0.29&0.08&176.5&0.30&0.09&140.3&
bar&0.52&0.18&174.0&0.56&0.19&53.2\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf ESO~443-80}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~479-4}}}\\
\multicolumn{7}{c}{Pec/RG? or SAB(s)m? }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO443-080.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO479-004.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RG&1.34&0.57&142.5&1.37&0.79&162.1&
r${\underline{\rm s}}$&0.84&0.49&59.3&0.92&0.83&72.1\\
&&&&&&&
bar&0.20&0.06&37.4&0.23&0.09&143.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~482-35}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~507-65}}}\\
\multicolumn{7}{c}{SB(rs)b }&
\multicolumn{7}{|c}{(R$^{\prime}$)Sm? }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO482-035.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO507-065.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.70&0.45&8.3&0.75&0.66&50.4&
R$^{\prime}$&0.77&0.24&16.8&0.77&0.56&3.4\\
bar&0.69&0.19&28.5&0.80&0.25&42.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~508-7}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~508-24}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(rs)d }&
\multicolumn{7}{|c}{SAB(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO508-007.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO508-024.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.59&0.39&111.8&0.91&0.48&72.9&
rs&0.60&0.35&72.9&0.60&0.41&167.3\\
bar&0.37&0.18&91.2&0.42&0.30&46.4&
bar&0.21&0.11&57.6&0.22&0.12&149.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf ESO~509-74}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~510-58}}}\\
\multicolumn{7}{c}{S(nd or nr)bc sp }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(s,nb)m or RG? }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO509-074.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO510-058.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
nr&0.14&0.03&136.2&0.14&0.12&151.3&
R$^{\prime}$&0.79&0.48&5.9&0.82&0.69&36.4\\
&&&&&&&
bar&0.35&0.23&161.1&0.38&0.31&128.9\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~510-59}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~532-22}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)c }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO510-059.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO532-022.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.59&0.51&127.8&0.89&0.54&82.3&
r${\underline{\rm s}}$&0.51&0.42&0.5&0.71&0.46&77.6\\
bar&0.33&0.07&116.2&0.41&0.09&49.8&
bar&0.45&0.13&17.3&0.63&0.13&70.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~545-16}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~547-5}}}\\
\multicolumn{7}{c}{(R)SAm }&
\multicolumn{7}{|c}{SAB(rs)m }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO545-016.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO547-005.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.54&1.39&36.9&1.79&1.54&89.5&
rs&0.66&0.42&52.1&0.66&0.57&7.1\\
&&&&&&&
bar&0.29&0.11&31.8&0.30&0.14&153.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf ESO~548-5}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~548-23}}}\\
\multicolumn{7}{c}{SAB(rs)dm }&
\multicolumn{7}{|c}{(RL:)SA0$^{-}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO548-005.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO548-023.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.73&0.56&53.7&0.73&0.65&19.9&
RL&0.66&0.35&24.3&0.68&0.66&70.0\\
bar&0.59&0.29&29.4&0.60&0.34&159.1&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~548-25}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~549-18}}}\\
\multicolumn{7}{c}{(R$^{\prime}$L)SB(s)a/d }&
\multicolumn{7}{|c}{(L,R$_{2}^{\prime}$)SAB(s)a/c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO548-025.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO549-018.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$L&0.90&0.41&81.5&0.92&0.77&154.2&
R$_{2}^{\prime}$&1.34&0.89&11.2&1.51&1.29&112.9\\
bar&0.25&0.13&172.2&0.47&0.13&88.2&
bar&0.66&0.22&16.8&0.66&0.36&175.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~572-18}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~576-1}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(rs)b: }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(r)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO572-018.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO576-001.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.67&0.27&45.4&0.70&0.52&27.4&
r&0.33&0.19&164.1&0.39&0.31&68.2\\
bar&0.27&0.15&178.7&0.43&0.19&109.4&
bar&0.21&0.14&32.7&0.38&0.15&79.2\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf ESO~576-3}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~576-32}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)dm }&
\multicolumn{7}{|c}{SB(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO576-003.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO576-032.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.04&0.24&93.4&1.05&0.61&169.0&
bar&0.69&0.17&153.2&0.73&0.23&26.7\\
&&&&&&&
rs&0.67&0.46&131.6&0.68&0.65&149.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~576-50}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~580-29}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{S(rs)b sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO576-050.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO580-029.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.75&0.39&166.4&0.84&0.56&137.4&
rs&0.76&0.09&71.6&0.77&0.49&168.2\\
bar&0.19&0.08&70.0&0.29&0.09&75.6&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf ESO~580-41}}}&
\multicolumn{7}{|c}{{\large{\bf ESO~581-25}}}\\
\multicolumn{7}{c}{SB:(r${\underline{\rm s}}$)dm sp }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$,nr?)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO580-041.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/ESO581-025.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.48&0.12&78.6&0.63&0.47&77.1&
r${\underline{\rm s}}$&1.03&0.12&59.2&1.03&0.62&176.8\\
&&&&&&&
nr&0.21&0.05&57.6&0.26&0.20&108.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf ESO~602-30}}}&
\multicolumn{7}{|c}{{\large{\bf IC~51}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)d }&
\multicolumn{7}{|c}{PRG }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/ESO602-030.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC0051.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.39&0.29&65.6&0.40&0.38&140.9&
PRG&0.50&0.10&113.9&$-$&$-$&$-$\\
bar&0.11&0.05&49.1&0.11&0.07&145.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~719}}}&
\multicolumn{7}{|c}{{\large{\bf IC~749}}}\\
\multicolumn{7}{c}{SA(rl)0$^{\rm o}$ }&
\multicolumn{7}{|c}{SB(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC0719.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC0749.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rl&0.28&0.06&51.8&0.28&0.14&4.5&
rs&0.70&0.60&53.1&0.78&0.61&106.4\\
&&&&&&&
bar&0.35&0.15&42.1&0.39&0.15&104.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~863}}}&
\multicolumn{7}{|c}{{\large{\bf IC~1014}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(rs)b }&
\multicolumn{7}{|c}{SB(r)m }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC0863.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC1014.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.51&0.30&44.1&0.51&0.40&167.6&
r&0.75&0.54&78.2&0.83&0.73&116.6\\
rs&0.24&0.22&76.6&0.30&0.24&78.7&
bar&0.37&0.16&54.2&0.43&0.20&130.3\\
bar&0.24&0.13&102.8&0.30&0.14&65.8&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf IC~1029}}}&
\multicolumn{7}{|c}{{\large{\bf IC~1048}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB$_{\rm a}$(s,nd)a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(s)d sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC1029.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC1048.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.30&0.33&147.6&2.34&1.41&167.1&
R$^{\prime}$&1.08&0.14&164.6&1.11&0.62&15.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~1055}}}&
\multicolumn{7}{|c}{{\large{\bf IC~1067}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(rs,r)ab }&
\multicolumn{7}{|c}{SB(r)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC1055.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC1067.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.53&0.54&5.7&1.54&1.33&6.3&
r&0.63&0.51&114.0&0.65&0.63&106.0\\
rs&0.90&0.28&3.2&0.91&0.69&170.7&
bar&0.61&0.22&150.0&0.67&0.25&41.4\\
r&0.33&0.13&7.6&0.34&0.31&42.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~1158}}}&
\multicolumn{7}{|c}{{\large{\bf IC~1210}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(${\underline{\rm r}}$s)cd }&
\multicolumn{7}{|c}{SAB(r)a: pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC1158.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC1210.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.31&0.17&141.2&0.33&0.29&39.9&
r&0.47&0.24&172.9&0.54&0.45&64.6\\
bar&0.17&0.10&81.8&0.26&0.11&105.7&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf IC~1265}}}&
\multicolumn{7}{|c}{{\large{\bf IC~1438}}}\\
\multicolumn{7}{c}{SA(r)0/a: }&
\multicolumn{7}{|c}{(R$_{1}$)SAB$_{\rm a}$(r$^{\prime}$l,nl)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC1265.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC1438.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.39&0.18&73.1&0.40&0.33&155.2&
R$_{1}$&1.77&1.32&23.4&1.86&1.40&48.6\\
&&&&&&&
r$^{\prime}$l&0.73&0.49&127.5&0.77&0.52&133.1\\
&&&&&&&
bar&0.70&0.34&123.4&0.74&0.36&132.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~1596}}}&
\multicolumn{7}{|c}{{\large{\bf IC~1953}}}\\
\multicolumn{7}{c}{SA(rs)bc: }&
\multicolumn{7}{|c}{SB(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC1596.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC1953.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.27&0.17&111.6&0.45&0.27&90.7&
bar&0.87&0.22&157.8&1.04&0.27&48.6\\
&&&&&&&
rs&0.77&0.70&100.8&1.07&0.76&95.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~1954}}}&
\multicolumn{7}{|c}{{\large{\bf IC~1993}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{(R$^{\prime}$)S${\underline{\rm A}}$B(s)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC1954.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC1993.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.48&0.25&77.3&0.56&0.39&50.6&
R$^{\prime}$&1.47&1.44&78.5&1.58&1.44&88.8\\
bar&0.13&0.05&91.6&0.17&0.07&52.3&
bar&0.54&0.39&43.8&0.56&0.40&56.2\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf IC~2051}}}&
\multicolumn{7}{|c}{{\large{\bf IC~2056}}}\\
\multicolumn{7}{c}{SB(${\underline{\rm r}}$s)b }&
\multicolumn{7}{|c}{SA(r${\underline{\rm s}}$)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC2051.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC2056.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.87&0.54&74.0&0.91&0.86&71.7&
r${\underline{\rm s}}$&0.27&0.23&114.5&0.31&0.24&94.5\\
bar&0.75&0.40&12.8&1.16&0.43&105.2&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~2361}}}&
\multicolumn{7}{|c}{{\large{\bf IC~2764}}}\\
\multicolumn{7}{c}{SA(r${\underline{\rm s}}$)bc }&
\multicolumn{7}{|c}{(R)SA(l)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC2361.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC2764.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.39&0.14&80.4&0.43&0.36&46.0&
R&0.84&0.70&3.3&0.84&0.82&9.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~2969}}}&
\multicolumn{7}{|c}{{\large{\bf IC~3102}}}\\
\multicolumn{7}{c}{SA(r)d }&
\multicolumn{7}{|c}{(R$^{\prime}$L)SAB(${\underline{\rm r}}$s)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC2969.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC3102.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.37&0.30&101.5&0.45&0.37&80.4&
R$^{\prime}$L&2.76&1.45&119.9&2.77&2.33&8.0\\
&&&&&&&
${\underline{\rm r}}$s&1.55&0.81&117.6&1.55&1.30&178.8\\
&&&&&&&
bar&0.78&0.38&128.0&0.81&0.59&27.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf IC~3267}}}&
\multicolumn{7}{|c}{{\large{\bf IC~3391}}}\\
\multicolumn{7}{c}{SA(rs)a }&
\multicolumn{7}{|c}{SA(r?)c pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC3267.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC3391.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.61&0.48&120.8&0.61&0.52&174.0&
r&0.23&0.13&50.6&0.24&0.17&150.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~3392}}}&
\multicolumn{7}{|c}{{\large{\bf IC~3806}}}\\
\multicolumn{7}{c}{SA(rs)ab }&
\multicolumn{7}{|c}{SA(r)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC3392.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC3806.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.58&0.25&39.3&0.60&0.56&47.4&
r&0.40&0.12&179.6&0.41&0.28&12.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~4214}}}&
\multicolumn{7}{|c}{{\large{\bf IC~4216}}}\\
\multicolumn{7}{c}{(R$_{1}$)S${\underline{\rm A}}$B$_{\rm a}$(r$^{\prime}$l,nr,nb)0/a }&
\multicolumn{7}{|c}{SB(r$^{\prime}$l=R$_{2}^{\prime}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC4214.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC4216.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{1}$&2.03&1.25&2.2&2.13&1.76&36.1&
r$^{\prime}$l&0.73&0.43&51.4&1.02&0.73&94.3\\
bar&0.90&0.42&150.0&1.00&0.57&141.4&
&&&&&&\\
r$^{\prime}$l&0.89&0.48&160.9&0.92&0.68&153.7&
&&&&&&\\
nr&0.21&0.13&165.2&0.21&0.19&141.4&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf IC~4221}}}&
\multicolumn{7}{|c}{{\large{\bf IC~4237}}}\\
\multicolumn{7}{c}{SB(${\underline{\rm r}}$s)dm }&
\multicolumn{7}{|c}{SB$_{\rm x}$(r)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC4221.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC4237.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.31&0.24&177.9&0.45&0.31&86.2&
r&0.57&0.39&152.3&0.60&0.53&49.8\\
bar&0.24&0.09&148.9&0.30&0.14&132.8&
bar&0.49&0.15&118.0&0.54&0.19&144.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~4536}}}&
\multicolumn{7}{|c}{{\large{\bf IC~4901}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{SB(r)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC4536.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC4901.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.66&0.64&68.5&0.76&0.65&84.2&
r&0.45&0.36&163.0&0.59&0.39&72.5\\
bar&0.45&0.12&169.1&0.46&0.14&154.8&
bar&0.41&0.18&119.0&0.42&0.25&172.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~5039}}}&
\multicolumn{7}{|c}{{\large{\bf IC~5156}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{SB$_{\rm a}$(r${\underline{\rm s}}$)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC5039.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC5156.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.31&0.17&158.6&0.51&0.31&85.3&
r${\underline{\rm s}}$&0.61&0.29&179.4&0.72&0.58&66.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf IC~5240}}}&
\multicolumn{7}{|c}{{\large{\bf IC~5264}}}\\
\multicolumn{7}{c}{SB$_{\rm x}$(r)0/a }&
\multicolumn{7}{|c}{(R)SA0$^{+}$ sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC5240.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC5264.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&1.33&0.36&89.7&1.34&0.51&166.6&
R&1.58&0.13&81.0&1.58&0.57&177.5\\
r&1.26&0.82&108.7&1.31&1.11&34.7&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~5267}}}&
\multicolumn{7}{|c}{{\large{\bf IC~5271}}}\\
\multicolumn{7}{c}{(RL)SA(r,l,nl)0/a }&
\multicolumn{7}{|c}{SAB(rs)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC5267.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/IC5271.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&4.65&3.31&148.4&4.80&4.33&38.4&
rs&1.07&0.39&138.8&1.07&1.02&22.3\\
r&2.71&1.95&136.3&2.74&2.61&151.0&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf IC~5334}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~24}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(l)0/a sp }&
\multicolumn{7}{|c}{S(rs)d: sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC5334.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0024.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.09&0.22&126.1&1.09&0.60&1.9&
rs&0.85&0.22&45.9&0.88&0.81&40.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~131}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~134}}}\\
\multicolumn{7}{c}{SAB(r${\underline{\rm s}}$)b: }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0131.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0134.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.83&0.23&64.8&0.83&0.64&10.8&
rs&1.26&0.34&45.5&1.30&1.18&146.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~148}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~150}}}\\
\multicolumn{7}{c}{(L)S${\underline{\rm A}}$B(r,nl)0$^{+}$ }&
\multicolumn{7}{|c}{SAB(r${\underline{\rm s}}$)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0148.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0150.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.70&0.19&88.9&0.71&0.49&4.3&
r${\underline{\rm s}}$&1.64&0.64&109.1&1.64&1.25&0.8\\
&&&&&&&
bar&0.62&0.23&51.3&1.08&0.26&105.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~210}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~244}}}\\
\multicolumn{7}{c}{(R$_{1}^{\prime}$,R2$^{\prime}$L)SAB(r$^{\prime}$l,nr)ab }&
\multicolumn{7}{|c}{(L)SA(rs:)m }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0210.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0244.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{2}^{\prime}$L&4.08&2.90&170.4&4.56&4.00&70.1&
rs&0.18&0.14&26.1&0.18&0.15&138.2\\
R$_{1}^{\prime}$&2.94&2.06&144.8&3.49&2.67&116.9&
&&&&&&\\
r$^{\prime}$l&1.47&0.88&169.9&1.51&1.32&30.8&
&&&&&&\\
bar&1.05&0.52&172.0&1.08&0.78&21.4&
&&&&&&\\
nr&0.20&0.14&155.5&0.22&0.19&112.7&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~253}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~254}}}\\
\multicolumn{7}{c}{SB(${\underline{\rm r}}$s)bc sp }&
\multicolumn{7}{|c}{(R)SAB(l)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0253.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0254.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&5.80&1.38&52.4&7.22&5.76&80.7&
R&1.59&1.25&139.5&1.91&1.57&79.9\\
&&&&&&&
bar&0.89&0.44&132.4&0.89&0.66&2.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~255}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~274}}}\\
\multicolumn{7}{c}{SB(rs)cd }&
\multicolumn{7}{|c}{(R)SA(l)0$^{-}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0255.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0274.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.74&0.53&62.0&0.81&0.53&71.7&
R&0.57&0.51&167.4&0.59&0.52&56.4\\
bar&0.20&0.07&57.4&0.22&0.07&64.9&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~289}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~470}}}\\
\multicolumn{7}{c}{(R:,R$^{\prime}$L)SA${\underline{\rm B}}$(rs$_{1}$,${\underline{\rm r}}$s$_{2}$)ab }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(r${\underline{\rm s}}$)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0289.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0470.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&6.07&4.68&139.9&7.19&5.79&69.9&
r${\underline{\rm s}}$&1.23&0.69&145.3&1.43&1.13&121.6\\
R$^{\prime}$L&3.00&2.18&117.6&3.26&2.95&111.6&
bar&0.76&0.34&12.0&1.10&0.45&62.5\\
rs&1.35&1.11&120.4&1.63&1.35&93.4&
&&&&&&\\
bar&0.69&0.26&125.4&0.69&0.38&3.1&
&&&&&&\\
${\underline{\rm r}}$s&0.66&0.63&43.2&0.97&0.63&91.1&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~473}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~474}}}\\
\multicolumn{7}{c}{(L)SA(r)0$^{+}$ }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(l)0/a (shells/ripples) }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0473.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0474.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.36&0.23&156.4&0.36&0.34&29.0&
R$^{\prime}$&2.23&2.07&67.2&2.28&2.21&62.5\\
&&&&&&&
bar&0.81&0.63&16.8&0.84&0.66&130.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~485}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~488}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)c }&
\multicolumn{7}{|c}{SA(rl)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0485.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0488.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.76&0.17&2.1&0.77&0.44&172.7&
rl&0.92&0.76&178.1&0.95&0.88&135.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~489}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~493}}}\\
\multicolumn{7}{c}{(R)S0$^{+}$ sp }&
\multicolumn{7}{|c}{SA(rs)d sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0489.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0493.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&0.67&0.08&121.3&0.67&0.30&2.3&
rs&0.96&0.24&53.7&1.01&0.77&150.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~532}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~600}}}\\
\multicolumn{7}{c}{SAB$_{\rm xa}$(r)0$^{+}$ }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0532.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0600.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.72&0.35&29.4&1.72&1.24&1.4&
r${\underline{\rm s}}$&1.07&0.76&76.0&1.09&0.81&35.4\\
&&&&&&&
bar&0.23&0.04&16.9&0.24&0.04&147.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~613}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~615}}}\\
\multicolumn{7}{c}{SB(${\underline{\rm r}}$s,nr)b }&
\multicolumn{7}{|c}{(R$_{2}^{\prime}$)S${\underline{\rm A}}$B$_{\rm x}$(${\underline{\rm r}}$l)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0613.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0615.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&2.90&0.70&123.3&2.90&0.90&176.6&
R$_{2}^{\prime}$&2.26&0.70&157.8&2.26&1.72&177.3\\
${\underline{\rm r}}$s&2.36&1.18&124.3&2.36&1.52&177.4&
${\underline{\rm r}}$l&0.69&0.21&159.0&0.69&0.51&3.2\\
nr&0.15&0.08&114.9&0.15&0.11&160.9&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~658}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~660}}}\\
\multicolumn{7}{c}{SA(r${\underline{\rm s}}$)bc }&
\multicolumn{7}{|c}{PRG }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0658.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0660.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.60&0.24&18.4&0.62&0.39&157.6&
PRG&5.98&1.33&175.5&$-$&$-$&$-$\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~672}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~676}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)d }&
\multicolumn{7}{|c}{SA(r)0$^{+}$ sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0672.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0676.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&3.51&1.34&69.1&3.51&2.93&1.4&
r&1.53&0.29&174.7&1.56&0.87&15.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~691}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~701}}}\\
\multicolumn{7}{c}{(R)SA(rs,r)ab }&
\multicolumn{7}{|c}{SB(${\underline{\rm r}}$s)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0691.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0701.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&2.74&1.93&98.8&2.79&2.55&29.0&
${\underline{\rm r}}$s&0.59&0.30&51.9&0.64&0.53&47.5\\
rs&1.67&1.06&98.6&1.68&1.41&17.0&
bar&0.21&0.06&63.0&0.24&0.10&37.4\\
r&1.03&0.75&89.5&1.04&1.00&151.7&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~718}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~723}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(rs,nl)a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(s)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0718.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0723.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.42&1.09&24.7&1.43&1.27&24.6&
R$^{\prime}$&0.45&0.40&151.2&0.45&0.41&179.0\\
rs&0.66&0.56&148.5&0.75&0.58&112.3&
&&&&&&\\
bar&0.66&0.39&154.4&0.72&0.42&129.7&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~755}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~779}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)d }&
\multicolumn{7}{|c}{(L)S${\underline{\rm A}}$B$_{\rm x}$(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0755.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0779.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.89&0.44&50.0&1.18&0.89&89.5&
rs&0.94&0.30&163.4&0.98&0.85&33.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~864}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~895}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)bc }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(${\underline{\rm r}}$s)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0864.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0895.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.17&0.83&59.2&1.46&0.97&64.8&
${\underline{\rm r}}$s&0.29&0.19&94.6&0.32&0.24&138.9\\
bar&0.87&0.37&104.8&1.27&0.37&83.1&
bar&0.14&0.08&158.9&0.17&0.09&64.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~908}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~936}}}\\
\multicolumn{7}{c}{SA(rs)b }&
\multicolumn{7}{|c}{(L)SB(${\underline{\rm r}}$s,bl)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0908.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0936.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.99&0.46&66.8&1.08&0.80&140.6&
${\underline{\rm r}}$s&1.55&1.22&139.8&1.71&1.49&64.1\\
&&&&&&&
bar&1.33&0.69&81.2&1.61&0.77&120.6\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~941}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~986}}}\\
\multicolumn{7}{c}{(R$^{\prime}$:)S${\underline{\rm A}}$B(r:)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(rs,nr:,nb)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0941.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC0986.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.11&1.52&169.4&2.15&2.08&54.4&
R$^{\prime}$&3.52&2.59&130.1&3.60&2.81&31.7\\
r&0.86&0.79&113.2&1.17&0.81&95.9&
bar&1.62&0.52&57.6&1.73&0.54&126.4\\
bar&0.33&0.17&13.7&0.37&0.21&43.4&
rs&1.56&1.05&51.5&1.69&1.08&117.2\\
&&&&&&&
nr&0.33&0.10&89.9&0.33&0.11&160.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1015}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1022}}}\\
\multicolumn{7}{c}{SB(r)0/a }&
\multicolumn{7}{|c}{(RL)SAB(${\underline{\rm r}}$s)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1015.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1022.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.81&0.67&17.7&0.81&0.77&22.7&
RL&2.08&1.66&143.7&2.13&1.74&138.1\\
bar&0.73&0.35&102.3&0.85&0.35&89.9&
${\underline{\rm r}}$s&0.94&0.87&59.0&1.00&0.88&76.3\\
&&&&&&&
bar&0.59&0.35&107.7&0.63&0.36&109.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1068}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1073}}}\\
\multicolumn{7}{c}{(R)SA(s,nr)a }&
\multicolumn{7}{|c}{SB(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1068.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1073.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&5.81&4.89&63.5&5.81&5.09&2.5&
rs&1.64&1.46&138.6&1.90&1.50&103.9\\
nr&0.56&0.48&51.9&0.56&0.50&166.9&
bar&1.59&0.43&61.1&1.77&0.46&55.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~1079}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1087}}}\\
\multicolumn{7}{c}{(L)S${\underline{\rm A}}$B$_{\rm a}$(${\underline{\rm r}}$s,bl)0$^{+}$ }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1079.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1087.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&1.36&0.75&86.8&1.42&1.18&32.8&
r${\underline{\rm s}}$&0.62&0.49&14.1&0.79&0.61&78.2\\
bar&1.01&0.51&119.5&1.37&0.62&62.7&
bar&0.50&0.22&128.5&0.71&0.25&111.9\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1090}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1097}}}\\
\multicolumn{7}{c}{SAB(s,nr$^{\prime}$l)bc }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(rs,nr)a${\underline{\rm b}}$ pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1090.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1097.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
nr$^{\prime}$l&0.26&0.10&93.7&0.27&0.21&155.4&
R$^{\prime}$&7.18&4.92&105.7&8.38&6.31&121.4\\
&&&&&&&
rs&3.44&2.03&136.9&3.60&2.91&33.2\\
&&&&&&&
bar&3.17&1.12&147.0&3.44&1.55&33.3\\
&&&&&&&
nr&0.34&0.29&167.3&0.47&0.31&80.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1163}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1179}}}\\
\multicolumn{7}{c}{SA(r:)0$^{+}$ sp }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1163.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1179.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.55&0.07&142.7&0.55&0.30&178.3&
r${\underline{\rm s}}$&1.18&1.10&46.0&1.33&1.18&92.0\\
&&&&&&&
bar&0.44&0.21&154.4&0.53&0.21&101.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~1187}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1232}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(rs)bc }&
\multicolumn{7}{|c}{SAB(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1187.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1232.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.59&0.76&115.5&1.60&1.02&167.4&
rs&0.78&0.51&92.2&0.78&0.59&177.0\\
bar&1.31&0.38&131.5&1.32&0.51&12.9&
bar&0.78&0.35&88.9&0.78&0.41&173.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1249}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1258}}}\\
\multicolumn{7}{c}{SB(rs:)m }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(s)a: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1249.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1258.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.80&0.65&75.0&1.96&1.42&142.7&
R$^{\prime}$&0.78&0.35&4.5&0.80&0.47&160.0\\
&&&&&&&
bar&0.31&0.21&83.3&0.42&0.21&77.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1291}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1297}}}\\
\multicolumn{7}{c}{(R)SAB(l,nb)0$^{+}$ }&
\multicolumn{7}{|c}{SA(rl,nl)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1291.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1297.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&8.47&7.08&69.6&8.51&7.10&53.1&
rl&0.76&0.72&174.1&0.78&0.75&121.4\\
bar&3.17&1.88&166.3&3.18&1.90&148.2&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~1300}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1302}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s,nrl)b }&
\multicolumn{7}{|c}{(RoRi)SAB(r)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1300.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1302.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&5.63&4.90&109.5&5.88&5.62&79.1&
R&3.19&2.98&17.8&3.20&3.09&13.0\\
bar&2.82&0.63&102.3&2.82&0.75&175.3&
R&2.19&1.95&60.7&2.24&1.98&57.7\\
nrl&0.15&0.14&114.0&0.17&0.15&84.0&
r&1.02&0.94&4.6&1.02&0.97&167.1\\
&&&&&&&
bar&0.93&0.62&169.4&0.93&0.64&155.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1310}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1326}}}\\
\multicolumn{7}{c}{SB(rs)cd }&
\multicolumn{7}{|c}{(R$_{1}$)SAB$_{\rm a}$(r,bl,nr)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1310.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1326.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.34&0.27&93.1&0.36&0.32&42.8&
R$_{1}$&2.83&1.87&85.9&2.84&2.34&12.2\\
bar&0.25&0.09&89.0&0.25&0.11&12.6&
r&1.09&0.89&63.2&1.18&1.04&120.9\\
&&&&&&&
bar&1.07&0.62&18.6&1.29&0.65&109.5\\
&&&&&&&
nr&0.18&0.16&61.9&0.20&0.18&112.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1341}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1350}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)d pec }&
\multicolumn{7}{|c}{(R)SAB$_{\rm a}$(r,bl)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1341.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1350.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.70&0.57&96.8&0.73&0.57&80.2&
R&5.35&2.60&179.5&5.56&4.75&147.5\\
bar&0.30&0.10&161.9&0.30&0.10&141.9&
r&2.25&1.15&14.1&2.49&1.97&47.4\\
&&&&&&&
bar&1.86&0.78&36.7&2.56&1.08&58.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~1353}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1357}}}\\
\multicolumn{7}{c}{SAB(rs,nl)a }&
\multicolumn{7}{|c}{(R$^{\prime}$L)SA(${\underline{\rm r}}$s)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1353.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1357.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.32&0.38&135.9&1.32&0.91&174.4&
R$^{\prime}$L&2.74&2.20&69.5&2.89&2.64&124.6\\
&&&&&&&
${\underline{\rm r}}$s&1.05&0.86&69.4&1.12&1.02&119.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1365}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1366}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(r${\underline{\rm s}}$,nr)bc }&
\multicolumn{7}{|c}{SA(rl)0$^{-}$ sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1365.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1366.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&10.56&5.03&41.4&11.08&8.15&29.6&
rl&0.38&0.15&1.9&0.38&0.34&177.5\\
bar&3.04&1.11&84.7&4.58&1.26&68.7&
&&&&&&\\
r${\underline{\rm s}}$&3.03&2.54&90.4&4.97&2.63&83.2&
&&&&&&\\
nr&0.30&0.18&15.6&0.35&0.26&124.6&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1367}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1385}}}\\
\multicolumn{7}{c}{(RL,RL)SAB(rs)0/a }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)dm pec /Sph }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1367.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1385.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&3.91&2.91&137.7&4.26&3.88&75.9&
r${\underline{\rm s}}$&0.68&0.60&39.5&0.99&0.63&82.6\\
RL&2.63&1.74&119.5&2.85&2.34&133.0&
bar&0.20&0.06&78.5&0.31&0.06&87.6\\
rs&1.32&0.94&131.9&1.36&1.32&107.7&
&&&&&&\\
bar&0.75&0.42&107.3&0.85&0.53&132.5&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~1386}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1398}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(r)0/a }&
\multicolumn{7}{|c}{(R)SB(${\underline{\rm r}}$s,bl)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1386.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1398.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.67&0.58&25.8&1.67&1.42&1.6&
R&4.64&3.17&87.7&4.70&4.22&156.8\\
r&0.50&0.20&24.8&0.51&0.49&157.2&
${\underline{\rm r}}$s&1.63&1.36&107.3&1.88&1.60&73.9\\
&&&&&&&
bar&1.33&0.83&13.4&1.78&0.84&95.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1415}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1425}}}\\
\multicolumn{7}{c}{(RL)SAB$_{\rm a}$(r$^{\prime}$l,nr)0$^{+}$ }&
\multicolumn{7}{|c}{(R$^{\prime}$R$^{\prime}$)SA(rl)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1415.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1425.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&4.10&1.35&157.4&4.29&3.21&27.0&
R$^{\prime}$&4.34&1.56&132.6&4.35&3.51&6.0\\
r$^{\prime}$l&1.60&0.51&145.1&1.72&1.18&147.8&
R$^{\prime}$&2.17&0.91&134.6&2.24&2.00&33.1\\
nr&0.24&0.11&164.0&0.32&0.22&63.4&
rl&0.65&0.30&137.1&0.73&0.61&57.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1433}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1436}}}\\
\multicolumn{7}{c}{(R$_{1}^{\prime}$)SB(r,nr,nb)a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(s)ab /Sph }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1433.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1436.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{1}^{\prime}$&6.26&4.48&14.3&6.31&5.17&162.3&
R$^{\prime}$&1.59&0.99&151.8&1.60&1.40&13.7\\
r&2.96&2.20&96.4&3.40&2.22&78.3&
bar&0.66&0.29&125.7&0.72&0.39&143.6\\
bar&2.87&1.00&95.2&3.29&1.01&74.0&
&&&&&&\\
nr&0.26&0.25&151.7&0.30&0.25&97.3&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~1438}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1448}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(r)0/a }&
\multicolumn{7}{|c}{SA(rs)c sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1438.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1448.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.05&0.48&70.7&1.06&1.00&21.1&
rs&1.36&0.19&42.5&1.36&0.97&177.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1452}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1483}}}\\
\multicolumn{7}{c}{(RL)SB(r,bl)0/a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(s)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1452.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1483.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&2.54&1.43&115.1&2.55&2.38&13.0&
R$^{\prime}$&0.83&0.55&141.0&0.85&0.66&28.3\\
r&1.63&0.91&113.7&1.63&1.53&179.8&
bar&0.60&0.20&2.9&0.70&0.21&63.5\\
bar&0.91&0.48&31.6&1.52&0.48&93.8&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1493}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1512}}}\\
\multicolumn{7}{c}{SB(rs)c }&
\multicolumn{7}{|c}{(RL)SB(r,nr)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1493.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1512.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.23&0.99&41.5&1.23&1.01&171.4&
RL&5.26&4.21&64.8&5.83&5.16&108.6\\
bar&0.89&0.34&78.0&0.90&0.34&29.0&
r&2.54&2.01&52.0&2.94&2.36&114.5\\
&&&&&&&
bar&2.45&0.84&44.4&2.72&1.03&139.1\\
&&&&&&&
nr&0.27&0.21&85.8&0.30&0.26&69.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~1515}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1532}}}\\
\multicolumn{7}{c}{(L)SA${\underline{\rm B}}$(${\underline{\rm r}}$s,nb$_{\rm a}$)0/a sp }&
\multicolumn{7}{|c}{SAB(rs,nd)ab sp pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1515.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1532.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&2.25&0.44&17.0&2.26&1.68&174.3&
rs&2.34&0.46&34.4&2.34&1.45&0.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1533}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1546}}}\\
\multicolumn{7}{c}{(RL)SB0$^{\rm o}$ }&
\multicolumn{7}{|c}{E(b)3/(R$^{\prime}$)SA(r)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1533.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1546.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&1.66&1.43&135.7&1.66&1.48&11.5&
R$^{\prime}$&0.96&0.40&150.8&0.99&0.87&33.8\\
bar&0.89&0.56&166.4&0.91&0.58&41.9&
r&0.53&0.17&148.0&0.53&0.39&2.9\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1553}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1566}}}\\
\multicolumn{7}{c}{SA(rl,nr$^{\prime}$l)0$^{+}$ }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$)SAB(r$^{\prime}$l,s,nb)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1553.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1566.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rl&1.18&0.67&150.6&1.18&0.93&174.3&
R$_{1}^{\prime}$&7.55&6.34&85.3&7.55&7.49&167.7\\
nr$^{\prime}$l&0.30&0.16&153.7&0.30&0.23&1.8&
r$^{\prime}$l&4.07&3.00&14.1&4.76&3.04&101.6\\
&&&&&&&
bar&3.94&2.35&12.6&4.61&2.38&102.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~1640}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~1672}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB$_{\rm a}$(r,bl)a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA${\underline{\rm B}}$(rs,nr)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1640.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1672.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.74&1.55&150.9&1.89&1.56&99.9&
R$^{\prime}$&4.89&3.84&163.7&4.95&4.24&26.0\\
bar&1.01&0.38&46.5&1.01&0.41&4.2&
bar&2.82&0.89&94.5&3.04&0.92&122.4\\
r&0.97&0.74&44.5&0.97&0.81&2.5&
rs&2.43&1.54&91.5&2.65&1.58&116.8\\
&&&&&&&
nr&0.22&0.17&124.3&0.23&0.19&143.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~1808}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2460}}}\\
\multicolumn{7}{c}{(R$_{1}$)SAB(s,nr)a }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC1808.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2460.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{1}$&6.38&4.62&130.5&6.52&6.18&42.2&
rs&0.37&0.29&21.3&0.45&0.34&110.1\\
bar&2.55&0.84&144.3&2.67&1.10&26.8&
&&&&&&\\
nr&0.24&0.14&138.8&0.25&0.18&26.1&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2550}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2552}}}\\
\multicolumn{7}{c}{(R)SAB(s)b pec }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(s)m }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2550.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2552.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&0.82&0.23&102.0&0.82&0.54&177.6&
R$^{\prime}$&1.88&1.22&53.6&1.96&1.67&35.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~2591}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2604}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)d sp }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$)SB(r${\underline{\rm s}}$)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2591.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2604.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.18&0.16&34.7&1.21&0.86&16.8&
R$_{1}^{\prime}$&0.88&0.57&146.2&1.01&0.57&97.1\\
&&&&&&&
bar&0.61&0.12&52.9&0.61&0.14&7.3\\
&&&&&&&
r${\underline{\rm s}}$&0.55&0.43&123.0&0.63&0.43&81.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2608}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2633}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)b }&
\multicolumn{7}{|c}{SAB(rs)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2608.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2633.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.33&0.60&70.1&1.53&0.74&46.9&
rs&0.66&0.32&173.9&0.69&0.49&155.5\\
bar&1.04&0.34&83.8&1.27&0.39&57.3&
bar&0.60&0.25&171.2&0.63&0.38&154.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2648}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2654}}}\\
\multicolumn{7}{c}{SA(r)a }&
\multicolumn{7}{|c}{SB$_{\rm x}$(r,nd)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2648.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2654.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.55&0.25&150.1&0.87&0.54&81.7&
r&1.17&0.17&64.6&1.17&0.63&178.5\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~2681}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2683}}}\\
\multicolumn{7}{c}{(R)S${\underline{\rm A}}$B(${\underline{\rm r}}$s)0/a }&
\multicolumn{7}{|c}{(RL)SB$_{\rm x}$(${\underline{\rm r}}$s)0/a sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2681.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2683.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&2.35&2.13&105.0&2.35&2.16&165.7&
RL&6.82&0.91&43.8&6.83&3.50&3.8\\
${\underline{\rm r}}$s&0.62&0.59&172.5&0.62&0.59&66.1&
${\underline{\rm r}}$s&3.34&0.39&43.3&3.34&1.48&0.8\\
bar&0.58&0.42&76.8&0.58&0.42&138.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2684}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2685}}}\\
\multicolumn{7}{c}{SA(rs)b }&
\multicolumn{7}{|c}{(R)S0$^{\rm o}$ PRG pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2684.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2685.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.38&0.34&35.7&0.42&0.38&105.4&
R&4.08&1.80&33.9&4.39&2.65&147.0\\
&&&&&&&
PRG&1.36&0.70&114.0&$-$&$-$&$-$\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2712}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2715}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(rs,nl)ab }&
\multicolumn{7}{|c}{SA(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2712.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2715.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.73&1.16&178.0&2.74&2.36&170.2&
rs&1.09&0.42&23.2&1.16&1.05&53.0\\
rs&0.85&0.52&175.3&1.07&0.84&98.5&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~2726}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2735}}}\\
\multicolumn{7}{c}{SB?(rs)0/a }&
\multicolumn{7}{|c}{SA:(r)0/a sp pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2726.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2735.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.47&0.13&87.3&0.47&0.34&175.3&
r&0.45&0.13&102.9&0.51&0.33&37.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2743}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2748}}}\\
\multicolumn{7}{c}{SB(rs)m }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(r)bc + PR? }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2743.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2748.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.33&0.25&96.9&0.39&0.32&106.6&
PRG&1.32&0.51&134.5&$-$&$-$&$-$\\
bar&0.25&0.10&123.8&0.26&0.15&31.0&
R$^{\prime}$&1.08&0.21&38.2&1.11&0.70&163.5\\
&&&&&&&
r&0.39&0.16&35.3&0.57&0.38&104.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2764}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2770}}}\\
\multicolumn{7}{c}{E(b)3/S(rs)a sp }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(rs)c sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2764.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2770.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.50&0.10&20.3&0.51&0.29&172.8&
rs&1.03&0.33&141.3&1.22&0.96&119.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~2775}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2780}}}\\
\multicolumn{7}{c}{SA(r,l)0$^{+}$ }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2775.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2780.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.42&1.06&157.2&1.44&1.30&160.4&
R$^{\prime}$&0.67&0.49&146.6&0.73&0.65&114.3\\
&&&&&&&
bar&0.41&0.10&115.5&0.49&0.12&129.8\\
&&&&&&&
rs&0.35&0.30&165.4&0.44&0.34&83.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2782}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2787}}}\\
\multicolumn{7}{c}{SA(rs,nr)a pec (shells/ripples)}&
\multicolumn{7}{|c}{(L)SB$_{\rm a}$(r,bl)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2782.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2787.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.01&0.87&81.8&1.10&0.95&117.7&
r&1.67&0.82&101.9&1.74&1.42&149.5\\
nr&0.15&0.11&80.8&0.17&0.13&133.6&
bar&0.93&0.60&147.6&1.41&0.72&71.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2793}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2805}}}\\
\multicolumn{7}{c}{RG pec }&
\multicolumn{7}{|c}{(R)S${\underline{\rm A}}$B(r${\underline{\rm s}}$)c pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2793.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2805.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RG&0.74&0.64&48.3&0.82&0.67&111.5&
R&1.60&1.26&152.1&1.69&1.52&51.4\\
&&&&&&&
r${\underline{\rm s}}$&0.53&0.36&90.5&0.63&0.39&115.5\\
&&&&&&&
bar&0.37&0.25&114.7&0.40&0.30&134.5\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~2841}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2844}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(r)a }&
\multicolumn{7}{|c}{SA(r)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2841.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2844.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&2.01&0.86&149.9&2.01&1.88&4.9&
r&0.28&0.12&10.3&0.28&0.21&169.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2854}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2859}}}\\
\multicolumn{7}{c}{SAB(r)a }&
\multicolumn{7}{|c}{(R)SAB$_{\rm a}$(rl,bl,nl,nb?)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2854.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2859.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.33&0.15&51.7&0.33&0.29&172.1&
R&3.42&2.73&85.5&3.48&3.38&47.9\\
bar&0.32&0.10&58.1&0.33&0.19&14.3&
rl&1.33&1.16&92.7&1.47&1.31&76.5\\
&&&&&&&
bar&1.13&0.71&161.6&1.41&0.71&83.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2882}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2893}}}\\
\multicolumn{7}{c}{SA(rs)b }&
\multicolumn{7}{|c}{(RL)SAB(l)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2882.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2893.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.62&0.30&77.4&0.64&0.60&143.0&
RL&0.87&0.69&58.4&0.88&0.73&11.6\\
&&&&&&&
bar&0.37&0.22&168.0&0.38&0.22&116.6\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~2894}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2903}}}\\
\multicolumn{7}{c}{(R:)SAB:0$^{-}$ }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(rs,nr)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2894.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2903.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.52&0.65&26.2&1.52&1.43&164.5&
R$^{\prime}$&10.12&3.62&19.5&10.12&7.44&179.5\\
&&&&&&&
rs&2.55&1.28&7.7&3.03&2.21&124.8\\
&&&&&&&
nr&0.16&0.09&24.2&0.19&0.16&70.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2906}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2962}}}\\
\multicolumn{7}{c}{SA(rs)ab or SA(rs)b /Sph }&
\multicolumn{7}{|c}{(R)S${\underline{\rm A}}$B$_{\rm a}$(rl)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2906.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2962.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.61&0.33&85.3&0.61&0.55&23.0&
R&2.13&1.42&7.5&2.18&2.12&108.1\\
&&&&&&&
bar&0.94&0.43&174.5&0.99&0.62&151.3\\
&&&&&&&
rl&0.93&0.55&2.7&0.95&0.82&155.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2964}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2966}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(r${\underline{\rm s}}$)b }&
\multicolumn{7}{|c}{(R$^{\prime}$?)SA${\underline{\rm B}}$(r$^{\prime}$l,nl)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2964.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2966.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.18&0.58&87.3&1.25&0.92&147.9&
R$^{\prime}$&2.34&1.69&46.0&2.34&2.09&8.2\\
bar&0.63&0.29&164.6&1.00&0.31&77.9&
r$^{\prime}$l&1.48&0.62&71.5&1.57&0.73&36.6\\
&&&&&&&
bar&1.45&0.42&76.4&1.56&0.48&40.1\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~2967}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2968}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(rs)c }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2967.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2968.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.55&1.43&126.4&1.61&1.44&71.6&
bar&1.18&0.65&39.9&1.31&0.80&134.9\\
rs&0.61&0.47&88.2&0.61&0.49&28.4&
r${\underline{\rm s}}$&1.14&0.75&43.1&1.28&0.93&130.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2974}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2985}}}\\
\multicolumn{7}{c}{SA(r)0/a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(r$^{\prime}$l)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2974.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2985.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.55&0.92&38.2&1.60&1.29&154.3&
R$^{\prime}$&3.34&2.13&1.3&3.36&2.69&13.6\\
&&&&&&&
r$^{\prime}$l&1.48&1.00&175.3&1.48&1.27&0.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3003}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3020}}}\\
\multicolumn{7}{c}{SB(rs)d }&
\multicolumn{7}{|c}{SB(rs)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3003.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3020.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.44&0.28&72.1&1.68&0.99&139.6&
rs&0.46&0.24&104.9&0.51&0.44&58.1\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3031}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3032}}}\\
\multicolumn{7}{c}{SA(rs,r,nb)a }&
\multicolumn{7}{|c}{SA(rl,l)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3031.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3032.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&6.45&3.29&148.7&6.88&5.68&139.9&
rl&0.61&0.54&90.2&0.68&0.61&98.3\\
r&4.30&2.07&157.4&4.30&3.80&6.8&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3041}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3061}}}\\
\multicolumn{7}{c}{SA(rs)b }&
\multicolumn{7}{|c}{SAB(${\underline{\rm r}}$s)b pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3041.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3061.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.15&0.81&84.8&1.30&1.14&104.6&
${\underline{\rm r}}$s&0.59&0.41&2.2&0.61&0.48&34.8\\
&&&&&&&
bar&0.35&0.15&158.7&0.35&0.18&174.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3066}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3147}}}\\
\multicolumn{7}{c}{SAB(rs)ab pec }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(r${\underline{\rm s}}$)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3066.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3147.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&0.44&0.20&91.6&0.46&0.21&135.1&
r${\underline{\rm s}}$&0.67&0.65&75.3&0.81&0.65&92.0\\
rs&0.41&0.37&39.5&0.45&0.37&88.8&
bar&0.64&0.51&136.3&0.66&0.59&134.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3153}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3166}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{(RL)SB$_{\rm a}$(rl)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3153.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3166.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.65&0.47&172.0&1.03&0.64&84.9&
RL&4.11&1.73&84.4&4.17&3.03&15.2\\
&&&&&&&
rl&0.92&0.66&89.8&1.21&0.90&78.8\\
&&&&&&&
bar&0.61&0.51&164.9&1.09&0.51&88.9\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3177}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3182}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(r${\underline{\rm s}}$)ab }&
\multicolumn{7}{|c}{SA(rl)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3177.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3182.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.63&0.43&130.8&0.63&0.49&169.7&
rl&0.19&0.16&132.4&0.20&0.19&91.8\\
r${\underline{\rm s}}$&0.24&0.17&27.9&0.27&0.17&75.7&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3184}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3185}}}\\
\multicolumn{7}{c}{SA(r${\underline{\rm s}}$)bc }&
\multicolumn{7}{|c}{(RL?)SAB$_{\rm ax}$(${\underline{\rm r}}$s)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3184.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3185.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.95&0.81&142.8&0.99&0.82&96.1&
RL&2.51&1.65&142.6&2.65&2.41&51.5\\
&&&&&&&
${\underline{\rm r}}$s&1.27&0.73&130.6&1.29&1.10&156.8\\
&&&&&&&
bar&1.13&0.45&114.6&1.25&0.62&142.6\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3198}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3248}}}\\
\multicolumn{7}{c}{SAB(r${\underline{\rm s}}$)bc }&
\multicolumn{7}{|c}{(RL)SA(l)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3198.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3248.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.85&0.40&40.1&1.99&1.12&27.5&
RL&1.77&1.10&117.8&1.79&1.77&125.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3259}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3266}}}\\
\multicolumn{7}{c}{SA(r$^{\prime}$l)bc }&
\multicolumn{7}{|c}{(RL)SB0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3259.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3266.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r$^{\prime}$l&0.27&0.15&23.9&0.28&0.26&41.2&
RL&0.79&0.60&86.2&0.79&0.66&170.9\\
&&&&&&&
bar&0.32&0.23&8.3&0.35&0.24&94.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3301}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3310}}}\\
\multicolumn{7}{c}{(RL)SAB$_{\rm x}$(r)0$^{+}$ sp }&
\multicolumn{7}{|c}{SA(${\underline{\rm r}}$s)bc pec (shells/ripples) }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3301.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3310.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&2.25&0.53&50.5&2.26&1.67&172.6&
${\underline{\rm r}}$s&0.30&0.19&130.7&0.31&0.21&139.9\\
r&0.99&0.28&53.7&1.01&0.87&26.3&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3319}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3321}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)cd }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(${\underline{\rm r}}$s)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3319.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3321.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&5.38&2.94&37.2&5.64&4.96&139.1&
${\underline{\rm r}}$s&0.54&0.34&14.0&0.76&0.50&107.9\\
bar&0.48&0.06&39.0&0.48&0.11&172.7&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3338}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3344}}}\\
\multicolumn{7}{c}{SA(rs,l)bc }&
\multicolumn{7}{|c}{SAB(r)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3338.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3344.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.68&0.42&92.5&0.87&0.67&98.7&
r&1.02&0.87&125.2&1.04&0.95&139.8\\
&&&&&&&
bar&0.84&0.52&4.5&0.89&0.55&49.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3346}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3351}}}\\
\multicolumn{7}{c}{SB(rs)cd }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(r,nr)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3346.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3351.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.63&0.43&149.6&0.68&0.47&46.9&
R$^{\prime}$&4.61&3.34&8.7&4.72&4.60&85.5\\
bar&0.50&0.14&93.7&0.52&0.17&152.9&
r&2.18&1.75&6.2&2.48&2.18&93.7\\
&&&&&&&
bar&2.01&1.08&112.5&2.81&1.10&98.3\\
&&&&&&&
nr&0.20&0.15&26.1&0.23&0.19&63.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3359}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3361}}}\\
\multicolumn{7}{c}{SB(rs)d }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3359.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3361.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.44&1.32&127.1&2.31&1.39&94.6&
rs&0.30&0.17&171.0&0.47&0.27&72.3\\
bar&0.62&0.12&15.7&0.77&0.16&47.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3368}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3380}}}\\
\multicolumn{7}{c}{(RL)SAB(${\underline{\rm r}}$s,nrl,nb)0$^{+}$ }&
\multicolumn{7}{|c}{(RL)SA${\underline{\rm B}}$(${\underline{\rm r}}$s)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3368.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3380.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&5.94&3.57&177.8&6.04&5.31&24.5&
RL&1.35&1.29&119.1&1.44&1.29&82.5\\
${\underline{\rm r}}$s&2.42&1.58&156.1&2.73&2.13&127.2&
bar&0.66&0.28&19.7&0.67&0.29&149.9\\
bar&2.09&1.20&125.0&2.82&1.35&113.2&
${\underline{\rm r}}$s&0.57&0.39&16.7&0.58&0.41&144.3\\
nrl&0.22&0.15&169.0&0.24&0.22&112.6&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3381}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3389}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)dm }&
\multicolumn{7}{|c}{SAB(r${\underline{\rm s}}$)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3381.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3389.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.61&0.54&61.6&0.65&0.61&81.0&
r${\underline{\rm s}}$&0.49&0.29&103.5&0.68&0.49&95.7\\
bar&0.59&0.13&75.6&0.60&0.16&22.3&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3403}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3437}}}\\
\multicolumn{7}{c}{SA(rs)bc: }&
\multicolumn{7}{|c}{SA(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3403.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3437.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.71&0.28&69.0&0.79&0.63&131.4&
rs&0.54&0.21&119.1&0.54&0.51&10.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3455}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3471}}}\\
\multicolumn{7}{c}{SA(rs:)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(s)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3455.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3471.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.36&0.22&63.5&0.41&0.36&85.7&
R$^{\prime}$&1.10&0.65&13.5&1.11&0.97&13.0\\
&&&&&&&
bar&0.09&0.03&32.9&0.10&0.04&35.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3485}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3486}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(${\underline{\rm r}}$s)b }&
\multicolumn{7}{|c}{SAB(r)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3485.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3486.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&0.91&0.25&45.8&0.93&0.26&32.1&
bar&0.76&0.33&75.3&0.77&0.44&166.5\\
${\underline{\rm r}}$s&0.70&0.61&58.9&0.72&0.63&57.3&
r&0.70&0.62&84.9&0.84&0.70&89.1\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3489}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3495}}}\\
\multicolumn{7}{c}{(R)SB(r:)0$^{\rm o}$ }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(rs)c: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3489.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3495.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.53&0.45&73.2&1.54&0.90&6.4&
R$^{\prime}$&3.05&0.58&20.1&3.06&2.18&171.6\\
r&0.71&0.58&39.7&1.25&0.66&97.3&
rs&1.01&0.30&20.6&1.12&1.01&99.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3504}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3507}}}\\
\multicolumn{7}{c}{(R$_{1}^{\prime}$)SA${\underline{\rm B}}$(${\underline{\rm r}}$s,nl)a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA${\underline{\rm B}}$(s)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3504.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3507.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{1}^{\prime}$&2.03&1.89&109.2&2.04&1.93&148.6&
R$^{\prime}$&2.34&2.11&75.8&2.44&2.34&101.3\\
${\underline{\rm r}}$s&1.18&0.65&154.7&1.18&0.67&24.6&
bar&0.79&0.34&109.3&0.82&0.38&34.6\\
bar&1.13&0.40&145.8&1.13&0.41&15.1&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3513}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3521}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)c }&
\multicolumn{7}{|c}{SA(rl,r)bc/E(b?)3 pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3513.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3521.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.82&0.67&64.0&0.83&0.81&135.1&
rl&1.97&0.89&156.1&2.16&1.79&131.3\\
bar&0.72&0.19&118.3&0.82&0.20&57.0&
r&0.83&0.27&160.0&0.83&0.59&170.6\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3547}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3556}}}\\
\multicolumn{7}{c}{SB(rs)cd }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3547.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3556.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.41&0.17&13.0&0.44&0.32&29.0&
r${\underline{\rm s}}$&3.87&0.86&80.6&3.87&2.94&179.3\\
bar&0.25&0.07&174.7&0.26&0.13&154.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3583}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3593}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(rs)a${\underline{\rm b}}$ }&
\multicolumn{7}{|c}{SA(r)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3583.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3593.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.96&1.04&118.7&2.00&1.30&159.6&
r&0.32&0.11&89.7&0.32&0.24&1.7\\
bar&0.71&0.29&77.4&0.85&0.31&117.6&
&&&&&&\\
rs&0.69&0.53&77.4&0.84&0.56&108.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3611}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3614}}}\\
\multicolumn{7}{c}{(R$^{\prime}$:)SA(r)a }&
\multicolumn{7}{|c}{SA(r)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3611.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3614.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.96&1.08&27.9&1.96&1.72&172.6&
r&0.47&0.24&70.9&0.63&0.32&119.9\\
r&0.17&0.12&17.8&0.20&0.17&113.5&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3623}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3625}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB$_{\rm x}$(rs)a }&
\multicolumn{7}{|c}{SB(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3623.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3625.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&5.85&1.32&172.5&5.90&4.65&166.7&
rs&0.37&0.15&155.5&0.40&0.35&52.8\\
rs&3.86&0.88&169.5&4.16&2.91&148.0&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3626}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3633}}}\\
\multicolumn{7}{c}{(RL,R)S${\underline{\rm A}}$B(rl,nl?)0/a }&
\multicolumn{7}{|c}{SA(r)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3626.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3633.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&2.35&1.55&166.8&2.37&2.22&26.1&
r&0.32&0.10&68.8&0.33&0.27&159.8\\
R&1.47&1.07&152.9&1.62&1.41&118.6&
&&&&&&\\
rl&0.69&0.47&160.6&0.70&0.67&139.0&
&&&&&&\\
bar&0.66&0.33&169.8&0.66&0.47&14.8&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3637}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3642}}}\\
\multicolumn{7}{c}{(RL)SB$_{\rm a}$(rl,bl)0$^{+}$ }&
\multicolumn{7}{|c}{SA(rl)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3637.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3642.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&1.44&1.12&133.7&1.44&1.25&171.9&
rl&0.42&0.40&105.1&0.44&0.42&85.4\\
rl&0.55&0.52&159.1&0.59&0.55&73.6&
&&&&&&\\
bar&0.49&0.33&35.7&0.55&0.33&80.5&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3664}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3673}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)m }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$$_{\rm x}$(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3664.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3673.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&1.42&0.27&40.1&1.65&0.30&125.5&
bar&1.47&0.38&84.3&1.50&0.62&14.1\\
r${\underline{\rm s}}$&1.34&1.26&80.2&1.62&1.34&92.4&
rs&1.42&0.74&77.7&1.42&1.22&4.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3675}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3681}}}\\
\multicolumn{7}{c}{(R$^{\prime}$,R$^{\prime}$)SA(s)b/E(d)4 }&
\multicolumn{7}{|c}{SAB(r,l)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3675.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3681.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.42&0.89&177.7&2.45&2.03&161.5&
r&0.60&0.51&159.8&0.63&0.53&55.8\\
R$^{\prime}$&1.62&0.54&179.4&1.62&1.25&174.3&
bar&0.26&0.16&154.8&0.27&0.18&38.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3682}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3683A}}}\\
\multicolumn{7}{c}{SA(r)0$^{+}$ }&
\multicolumn{7}{|c}{SAB(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3682.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3683A.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.20&0.13&98.0&0.21&0.19&41.5&
rs&0.46&0.24&67.8&0.47&0.36&8.5\\
&&&&&&&
bar&0.18&0.11&76.7&0.19&0.15&33.5\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3684}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3687}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(s)c }&
\multicolumn{7}{|c}{(RL)SA${\underline{\rm B}}$(rs)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3684.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3687.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.52&0.98&114.6&1.56&1.42&147.8&
RL&1.43&1.34&164.6&1.49&1.35&108.7\\
bar&0.36&0.17&128.5&0.37&0.24&17.3&
rs&0.44&0.41&123.7&0.46&0.41&85.5\\
&&&&&&&
bar&0.43&0.21&174.8&0.44&0.22&130.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3689}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3691}}}\\
\multicolumn{7}{c}{SA(r)b }&
\multicolumn{7}{|c}{SB(r)m }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3689.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3691.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.24&0.13&94.3&0.24&0.21&15.6&
r&0.75&0.51&11.4&0.77&0.65&150.9\\
&&&&&&&
bar&0.70&0.17&31.2&0.71&0.22&13.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3692}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3701}}}\\
\multicolumn{7}{c}{(R$^{\prime}$L)SA(r)0/a sp }&
\multicolumn{7}{|c}{SA(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3692.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3701.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$L&1.81&0.40&92.9&1.83&1.59&163.4&
rs&0.26&0.15&155.7&0.33&0.24&67.8\\
r&0.68&0.15&94.0&0.68&0.61&2.7&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3705}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3715}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(${\underline{\rm r}}$s)b }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rs)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3705.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3715.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.53&1.06&119.6&2.54&2.00&4.8&
rs&0.32&0.27&112.0&0.35&0.30&119.6\\
${\underline{\rm r}}$s&1.17&0.49&121.8&1.18&0.92&13.3&
bar&0.25&0.18&75.8&0.30&0.18&108.1\\
bar&0.42&0.37&65.5&0.77&0.38&94.9&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3718}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3726}}}\\
\multicolumn{7}{c}{SAB(r,l,nl)a pec }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(r)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3718.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3726.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&2.91&2.14&154.3&6.29&2.57&98.2&
r&1.50&0.84&12.1&1.54&1.31&154.0\\
&&&&&&&
bar&1.38&0.30&30.2&1.43&0.47&20.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3729}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3730}}}\\
\multicolumn{7}{c}{(L)SB(r)0/a + dwarf comp. }&
\multicolumn{7}{|c}{SA(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3729.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3730.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.25&0.59&160.4&1.28&0.80&158.1&
rs&0.21&0.18&94.9&0.21&0.19&32.6\\
bar&0.70&0.24&25.3&0.80&0.30&45.5&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3735}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3755}}}\\
\multicolumn{7}{c}{SAB(rs)c: sp }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA${\underline{\rm B}}$(s)c pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3735.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3755.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.79&0.15&130.7&0.80&0.64&18.8&
R$^{\prime}$&2.64&0.97&130.3&2.71&2.59&52.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3769}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3780}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)cd }&
\multicolumn{7}{|c}{SA(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3769.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3780.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.98&0.30&145.5&1.07&0.87&136.8&
rs&0.48&0.27&77.5&0.48&0.35&171.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3782}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3786}}}\\
\multicolumn{7}{c}{SB(rs)dm }&
\multicolumn{7}{|c}{(R)SA(r)0/a pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3782.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3786.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.93&0.47&175.2&0.94&0.57&170.3&
R&1.77&0.79&75.1&1.79&1.43&17.4\\
bar&0.45&0.12&172.6&0.45&0.14&168.3&
r&0.85&0.40&69.4&0.85&0.73&171.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3788}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3835}}}\\
\multicolumn{7}{c}{SA(r)a }&
\multicolumn{7}{|c}{(L)SA(${\underline{\rm r}}$s)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3788.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3835.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.44&0.14&0.3&0.61&0.42&72.2&
${\underline{\rm r}}$s&0.51&0.16&58.8&0.51&0.48&9.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3870}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3876}}}\\
\multicolumn{7}{c}{SB(rs)0$^{\rm o}$? }&
\multicolumn{7}{|c}{Ring pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3870.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3876.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.66&0.55&28.9&0.76&0.66&82.8&
RG&0.56&0.39&110.0&0.68&0.55&74.0\\
bar&0.32&0.14&29.8&0.32&0.19&12.1&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3885}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3887}}}\\
\multicolumn{7}{c}{(L)S${\underline{\rm A}}$B(r${\underline{\rm l}}$,nl)0$^{+}$ }&
\multicolumn{7}{|c}{(RL)SA${\underline{\rm B}}$$_{\rm x}$(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3885.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3887.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm l}}$&0.66&0.32&126.6&0.78&0.63&65.7&
RL&3.38&2.33&9.9&3.42&2.74&158.3\\
&&&&&&&
bar&1.13&0.33&1.9&1.16&0.39&155.7\\
&&&&&&&
rs&1.13&0.82&174.0&1.20&0.92&134.8\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3888}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3892}}}\\
\multicolumn{7}{c}{SA(rs)b }&
\multicolumn{7}{|c}{(RL)SA${\underline{\rm B}}$(r$^{\prime}$l)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3888.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3892.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.42&0.30&129.6&0.43&0.39&41.2&
RL&2.55&2.20&4.0&2.66&2.20&85.5\\
&&&&&&&
r$^{\prime}$l&1.16&0.91&92.6&1.16&0.94&171.5\\
&&&&&&&
bar&1.13&0.60&100.5&1.13&0.63&0.9\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3898}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3900}}}\\
\multicolumn{7}{c}{(RR)SA0$^{+}$ }&
\multicolumn{7}{|c}{SA(r)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3898.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3900.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&2.38&0.84&104.0&2.40&1.48&170.1&
r&1.10&0.43&179.7&1.10&0.79&171.7\\
R&1.80&0.65&106.2&1.81&1.14&175.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3936}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3941}}}\\
\multicolumn{7}{c}{SA(rs)c sp }&
\multicolumn{7}{|c}{(R)SB$_{\rm a}$0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3936.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3941.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.42&0.12&64.5&0.77&0.42&89.2&
R&1.78&0.94&3.9&1.80&1.47&164.0\\
&&&&&&&
bar&0.70&0.39&174.9&0.76&0.57&141.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3949}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3953}}}\\
\multicolumn{7}{c}{SAB(r${\underline{\rm s}}$)c }&
\multicolumn{7}{|c}{SB(r)${\underline{\rm b}}$c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3949.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3953.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.67&0.33&117.3&0.68&0.53&164.6&
r&1.60&0.73&6.6&1.68&1.33&147.0\\
bar&0.19&0.10&113.5&0.20&0.17&143.2&
bar&0.91&0.42&47.3&1.29&0.57&61.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3955}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3956}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)bc/S0$^{-}$ /Sph }&
\multicolumn{7}{|c}{SAB(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3955.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3956.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.66&0.16&173.3&0.71&0.42&30.0&
rs&0.78&0.21&54.7&0.93&0.57&134.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3976}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3982}}}\\
\multicolumn{7}{c}{SAB(rs)${\underline{\rm b}}$c }&
\multicolumn{7}{|c}{SA(rs)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3976.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3982.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.85&0.22&58.6&0.85&0.67&7.8&
rs&0.47&0.42&64.8&0.51&0.44&69.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~3985}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~3992}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)m }&
\multicolumn{7}{|c}{SB(rs,nb)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3985.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3992.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.24&0.20&91.9&0.27&0.23&74.0&
rs&2.73&1.69&73.4&2.99&2.70&72.7\\
bar&0.15&0.09&139.5&0.19&0.09&73.0&
bar&1.80&0.69&38.5&2.32&0.94&126.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~3998}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4027}}}\\
\multicolumn{7}{c}{SA(r)0$^{\rm o}$ }&
\multicolumn{7}{|c}{SB(rs)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC3998.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4027.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.21&1.01&139.1&1.26&1.20&73.9&
rs&0.65&0.56&102.3&0.79&0.57&98.6\\
&&&&&&&
bar&0.22&0.06&87.0&0.28&0.06&94.9\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4030}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4037}}}\\
\multicolumn{7}{c}{SA(rs)bc }&
\multicolumn{7}{|c}{SAB(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4030.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4037.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.43&0.31&34.7&0.44&0.40&21.7&
bar&1.08&0.40&13.3&1.13&0.44&37.1\\
&&&&&&&
rs&0.91&0.85&105.0&1.05&0.86&100.1\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4041}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4045}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(rs)c }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$L)SAB(${\underline{\rm r}}$s,nl)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4041.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4045.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.35&0.30&83.6&0.37&0.31&55.9&
R$_1^{\prime}$L&1.91&0.95&89.1&1.91&1.43&3.2\\
bar&0.20&0.10&74.5&0.21&0.10&37.0&
${\underline{\rm r}}$s&0.65&0.48&85.2&0.73&0.65&96.8\\
&&&&&&&
bar&0.54&0.33&17.9&0.80&0.34&100.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4050}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4051}}}\\
\multicolumn{7}{c}{(RL)SA${\underline{\rm B}}$(${\underline{\rm r}}$s)a }&
\multicolumn{7}{|c}{SAB(rs)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4050.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4051.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&3.36&2.01&88.8&3.38&3.03&165.9&
bar&2.22&0.59&132.1&2.23&0.68&11.6\\
${\underline{\rm r}}$s&2.02&1.33&90.1&2.04&1.99&142.6&
rs&2.07&1.32&115.9&2.07&1.53&170.3\\
bar&1.81&0.54&77.8&1.89&0.78&157.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4062}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4064}}}\\
\multicolumn{7}{c}{SA(rs)b }&
\multicolumn{7}{|c}{(RL)SB(ls)0$^{\rm o}$/d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4062.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4064.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.72&0.37&107.6&0.98&0.69&72.4&
RL&3.27&1.16&148.2&3.27&2.46&176.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4067}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4094}}}\\
\multicolumn{7}{c}{SB(rs)ab }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(s)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4067.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4094.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.38&0.33&45.3&0.44&0.38&89.0&
R$^{\prime}$&1.74&0.64&55.8&2.03&1.47&130.4\\
bar&0.37&0.17&61.7&0.38&0.21&27.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4100}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4102}}}\\
\multicolumn{7}{c}{(R$^{\prime}$L)S${\underline{\rm A}}$B(rs,nr?)ab sp }&
\multicolumn{7}{|c}{(R$^{\prime}$)S${\underline{\rm A}}$B$_{\rm a}$(l)ab /Sph }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4100.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4102.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$L&4.65&1.48&166.1&4.80&4.36&36.1&
R$^{\prime}$&1.24&0.67&42.8&1.27&1.19&42.1\\
rs&0.94&0.29&155.0&1.14&0.72&131.7&
bar&0.44&0.27&57.9&0.55&0.38&62.7\\
nr&0.12&0.05&151.7&0.18&0.10&110.2&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4108}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4108B}}}\\
\multicolumn{7}{c}{SAB(rs)c }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4108.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4108B.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.26&0.17&97.0&0.26&0.21&4.2&
rs&0.29&0.22&114.8&0.32&0.24&125.0\\
bar&0.13&0.08&101.4&0.13&0.09&11.0&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4116}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4120}}}\\
\multicolumn{7}{c}{SB(rs)d }&
\multicolumn{7}{|c}{SB(rs:)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4116.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4120.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.58&1.00&135.4&1.88&1.51&111.8&
rs&0.42&0.20&168.9&0.68&0.42&88.6\\
bar&1.52&0.43&142.7&1.53&0.76&175.2&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4123}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4136}}}\\
\multicolumn{7}{c}{SB$_{\rm x}$(rs)b }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4123.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4136.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&1.75&0.42&106.1&1.84&0.59&155.0&
rs&0.68&0.50&92.4&0.74&0.52&57.9\\
rs&1.61&1.05&114.4&1.68&1.47&141.1&
bar&0.49&0.23&22.9&0.50&0.25&154.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4138}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4141}}}\\
\multicolumn{7}{c}{SA(r)0$^{+}$ }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4138.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4141.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.74&0.40&154.3&0.76&0.68&35.8&
r${\underline{\rm s}}$&0.38&0.28&57.2&0.41&0.34&125.9\\
&&&&&&&
bar&0.24&0.11&86.2&0.25&0.15&17.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4145}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4152}}}\\
\multicolumn{7}{c}{SAB(rs)d }&
\multicolumn{7}{|c}{SAB(r${\underline{\rm s}}$)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4145.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4152.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.79&0.35&81.1&0.88&0.55&141.6&
r${\underline{\rm s}}$&0.32&0.27&93.5&0.38&0.30&107.1\\
bar&0.36&0.16&135.6&0.49&0.20&60.9&
bar&0.17&0.11&40.9&0.22&0.11&94.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4158}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4162}}}\\
\multicolumn{7}{c}{(RL)SAB$_{\rm a}$(r)a }&
\multicolumn{7}{|c}{SA(r)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4158.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4162.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&0.62&0.44&68.5&0.62&0.57&5.0&
r&0.37&0.22&166.8&0.37&0.34&161.7\\
r&0.30&0.21&77.4&0.31&0.27&32.4&
&&&&&&\\
bar&0.23&0.13&52.0&0.24&0.17&151.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4178}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4189}}}\\
\multicolumn{7}{c}{(R$_{2}^{\prime}$)SB(s)d }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4178.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4189.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{2}^{\prime}$&3.53&1.07&31.3&3.81&3.51&101.7&
bar&0.84&0.24&102.5&0.91&0.28&38.7\\
&&&&&&&
r${\underline{\rm s}}$&0.73&0.58&109.5&0.86&0.64&66.1\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4192}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4193}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB$_{\rm x}$(rs,nd)a }&
\multicolumn{7}{|c}{(RL)SAB(r${\underline{\rm s}}$)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4192.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4193.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&7.96&1.67&155.5&7.97&5.39&175.6&
RL&1.75&0.79&88.3&1.75&1.71&159.0\\
rs&4.10&0.81&151.2&4.32&2.47&156.4&
r${\underline{\rm s}}$&0.44&0.28&95.5&0.63&0.43&82.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4210}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4212}}}\\
\multicolumn{7}{c}{SB(rs)bc }&
\multicolumn{7}{|c}{SA(rs)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4210.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4212.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.47&0.33&123.0&0.54&0.39&55.8&
rs&0.72&0.40&76.5&0.72&0.61&6.2\\
bar&0.38&0.16&45.4&0.46&0.17&121.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4216}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4220}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB$_{\rm box,a}$(r,nd)a }&
\multicolumn{7}{|c}{(L)SAB(r)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4216.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4220.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&5.84&0.55&20.9&5.85&3.02&3.9&
r&1.17&0.21&137.8&1.17&0.70&172.7\\
r&1.86&0.26&19.2&1.89&1.42&165.5&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4224}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4234}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA0$^{+}$ }&
\multicolumn{7}{|c}{(L)SB(rs)m }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4224.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4234.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.44&0.28&57.8&1.45&0.70&9.4&
bar&0.64&0.11&78.3&0.67&0.13&33.5\\
&&&&&&&
rs&0.54&0.37&71.3&0.56&0.43&37.9\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4237}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4245}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(s)b }&
\multicolumn{7}{|c}{(RL)SB(r,nr)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4237.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4245.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.14&0.71&105.8&1.15&1.14&37.5&
RL&2.65&1.89&16.6&2.72&2.20&30.5\\
&&&&&&&
bar&1.25&0.61&136.5&1.38&0.66&128.1\\
&&&&&&&
r&1.21&0.90&151.8&1.30&1.01&132.4\\
&&&&&&&
nr&0.16&0.13&176.3&0.16&0.15&168.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4250}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4256}}}\\
\multicolumn{7}{c}{(R)SAB(rl,nl!)0$^{+}$ }&
\multicolumn{7}{|c}{(R)S0$^{+}$ sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4250.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4256.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&3.10&2.68&83.8&3.19&2.96&133.1&
R&2.37&0.20&41.6&2.37&1.10&0.3\\
rl&1.43&1.01&166.5&1.60&1.02&73.7&
&&&&&&\\
bar&1.43&0.60&165.1&1.60&0.61&69.8&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4258}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4260}}}\\
\multicolumn{7}{c}{(R)SAB(rs,nb or nd$_{\rm sp}$)a }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4258.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4260.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&16.51&5.47&146.6&23.39&15.26&69.9&
r${\underline{\rm s}}$&1.12&0.62&57.9&1.61&1.12&89.4\\
rs&6.33&2.03&155.7&10.90&4.66&66.2&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4268}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4274}}}\\
\multicolumn{7}{c}{SA:(${\underline{\rm r}}$s)0$^{+}$ sp }&
\multicolumn{7}{|c}{(R)SB(r,nr)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4268.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4274.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.66&0.21&48.6&0.67&0.42&13.6&
R&5.92&1.50&100.8&5.93&4.41&177.3\\
&&&&&&&
r&2.79&0.91&100.3&2.81&2.66&155.6\\
&&&&&&&
nr&0.26&0.08&102.7&0.26&0.24&29.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4286}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4293}}}\\
\multicolumn{7}{c}{d(R${\underline{\rm L}}$)SA(l)0$^{\rm o}$,N /Sph }&
\multicolumn{7}{|c}{(R)SB$_{\rm x}$(rs)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4286.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4293.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R{\underline{\rm L}}&0.78&0.55&160.2&0.91&0.77&74.3&
R&4.20&2.11&64.4&4.51&4.19&86.2\\
&&&&&&&
rs&2.49&0.99&72.8&2.71&1.96&36.5\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4298}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4303}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(rs)bc }&
\multicolumn{7}{|c}{SAB(rs,nl)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4298.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4303.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.13&0.96&138.3&2.20&1.62&22.8&
bar&1.86&0.56&2.1&1.95&0.60&42.4\\
rs&0.71&0.25&132.5&0.71&0.43&3.4&
rs&1.59&1.33&81.0&1.76&1.35&106.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4309}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4310}}}\\
\multicolumn{7}{c}{SAB(rl)0$^{\rm o}$ }&
\multicolumn{7}{|c}{SA(${\underline{\rm r}}$s)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4309.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4310.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rl&0.99&0.37&90.5&1.00&0.68&172.5&
${\underline{\rm r}}$s&0.43&0.14&157.2&0.43&0.30&177.0\\
bar&0.66&0.34&73.9&0.80&0.52&126.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4313}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4314}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)0/a sp }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$)SB(rl,nr)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4313.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4314.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.40&0.20&142.0&1.41&0.87&4.5&
R$_{1}^{\prime}$&3.72&3.03&51.2&3.72&3.23&179.4\\
&&&&&&&
bar&2.22&0.80&146.9&2.37&0.80&94.9\\
&&&&&&&
rl&2.07&1.74&155.1&2.20&1.74&99.8\\
&&&&&&&
nr&0.23&0.18&140.0&0.25&0.18&88.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4316}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4319}}}\\
\multicolumn{7}{c}{SB(rs?)c sp }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA${\underline{\rm B}}$(${\underline{\rm r}}$s)a pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4316.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4319.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.95&0.06&111.9&0.95&0.39&2.1&
R$^{\prime}$&2.16&1.69&168.0&2.32&2.00&53.9\\
&&&&&&&
${\underline{\rm r}}$s&1.12&0.61&134.4&1.16&0.76&154.5\\
&&&&&&&
bar&0.60&0.30&162.8&0.61&0.37&19.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4321}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4324}}}\\
\multicolumn{7}{c}{SAB(r${\underline{\rm s}}$,nr)bc }&
\multicolumn{7}{|c}{(L)SA(r)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4321.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4324.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&2.22&0.90&107.9&2.52&0.96&122.5&
r&0.72&0.32&54.0&0.75&0.71&119.1\\
r${\underline{\rm s}}$&2.03&1.70&103.0&2.38&1.75&106.3&
&&&&&&\\
nr&0.30&0.24&158.6&0.30&0.29&1.6&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4336}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4343}}}\\
\multicolumn{7}{c}{SAB(r)0/a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB$_{\rm x}$(r)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4336.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4343.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.59&0.32&167.0&0.60&0.53&26.8&
R$^{\prime}$&0.92&0.14&127.5&0.93&0.41&171.3\\
bar&0.28&0.18&101.7&0.45&0.19&102.2&
r&0.45&0.10&132.9&0.46&0.28&12.6\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4344}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4348}}}\\
\multicolumn{7}{c}{dSA(r)0$^{+}$ ,N }&
\multicolumn{7}{|c}{SB(rs)bc sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4344.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4348.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.31&0.27&155.8&0.35&0.27&94.8&
rs&0.68&0.14&33.8&0.71&0.58&151.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4351}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4355}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)S${\underline{\rm A}}$B(s)dm imbedded }&
\multicolumn{7}{|c}{(R$^{\prime}$L)S${\underline{\rm A}}$B(l)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4351.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4355.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.25&0.83&76.9&1.38&1.11&51.4&
R$^{\prime}$L&0.97&0.49&60.1&1.01&0.95&129.5\\
&&&&&&&
bar&0.63&0.32&61.6&0.63&0.62&127.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4369}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4371}}}\\
\multicolumn{7}{c}{(R)SB(rs)0/a: pec }&
\multicolumn{7}{|c}{(L)SB$_{\rm a}$(r,nr)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4369.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4371.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.42&1.30&156.8&1.45&1.31&62.2&
r&2.09&1.04&91.1&2.14&1.97&35.1\\
rs&0.28&0.25&105.6&0.28&0.26&5.9&
bar&1.13&0.84&158.0&2.13&0.86&84.7\\
bar&0.27&0.10&150.5&0.27&0.10&50.2&
nr&0.35&0.14&87.3&0.35&0.27&177.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4378}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4380}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(l)a }&
\multicolumn{7}{|c}{(R)SA(r,l)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4378.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4380.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.93&2.45&178.5&2.99&2.85&43.2&
R&2.02&1.07&156.5&2.03&1.93&169.8\\
&&&&&&&
r&0.98&0.54&151.8&1.04&0.92&132.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4384}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4385}}}\\
\multicolumn{7}{c}{(L)SB(rs)dm }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(rs)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4384.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4385.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.30&0.15&75.5&0.30&0.20&168.3&
rs&1.03&0.60&84.7&1.10&0.96&46.6\\
bar&0.07&0.04&157.9&0.09&0.04&80.3&
bar&0.97&0.37&99.4&1.12&0.55&41.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4388}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4389}}}\\
\multicolumn{7}{c}{SA:(rs)a sp }&
\multicolumn{7}{|c}{SB(${\underline{\rm r}}$s)0/a/d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4388.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4389.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.39&0.17&89.3&1.40&0.62&172.4&
${\underline{\rm r}}$s&1.50&0.75&101.9&1.52&1.16&15.7\\
&&&&&&&
bar&1.38&0.25&104.6&1.40&0.38&13.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4394}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4402}}}\\
\multicolumn{7}{c}{(R)SB(${\underline{\rm r}}$s,nl)0/a }&
\multicolumn{7}{|c}{(R$^{\prime}$)S${\underline{\rm A}}$B(s)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4394.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4402.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&2.74&2.45&77.5&2.99&2.60&113.0&
R$^{\prime}$&1.86&0.20&89.8&1.95&1.28&23.2\\
bar&1.52&0.65&142.2&1.60&0.72&38.3&
&&&&&&\\
${\underline{\rm r}}$s&1.50&1.31&129.2&1.58&1.44&58.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4405}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4411A}}}\\
\multicolumn{7}{c}{(R)SA${\underline{\rm B}}$(${\underline{\rm r}}$s)a }&
\multicolumn{7}{|c}{SB(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4405.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4411A.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.05&0.66&24.2&1.05&0.87&13.3&
rs&0.57&0.43&32.6&0.68&0.43&94.5\\
${\underline{\rm r}}$s&0.37&0.32&13.8&0.42&0.37&96.4&
bar&0.16&0.03&109.7&0.16&0.03&173.4\\
bar&0.34&0.14&7.9&0.34&0.18&163.6&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4412}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4413}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)bc }&
\multicolumn{7}{|c}{(R$^{\prime}$L)SB(${\underline{\rm r}}$s)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4412.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4413.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.73&0.56&77.9&0.73&0.58&24.3&
R$^{\prime}$L&2.81&1.52&68.5&2.81&2.14&178.2\\
bar&0.54&0.16&119.7&0.56&0.16&63.5&
${\underline{\rm r}}$s&1.28&0.64&58.6&1.31&0.88&159.1\\
&&&&&&&
bar&0.49&0.24&14.2&0.64&0.26&112.6\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4414}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4416}}}\\
\multicolumn{7}{c}{SA(rl)bc }&
\multicolumn{7}{|c}{(RL)SB(rs)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4414.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4416.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rl&0.68&0.39&145.2&0.82&0.60&122.0&
RL&1.08&1.01&98.4&1.17&1.07&82.4\\
&&&&&&&
rs&0.41&0.32&66.6&0.43&0.36&139.6\\
&&&&&&&
bar&0.19&0.06&7.5&0.22&0.06&97.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4424}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4430}}}\\
\multicolumn{7}{c}{(R$_{2}^{\prime}$L)SB(s)0/a pec }&
\multicolumn{7}{|c}{SAB(${\underline{\rm r}}$s)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4424.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4430.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{2}^{\prime}$L&3.18&1.53&89.9&3.25&2.70&22.5&
${\underline{\rm r}}$s&0.56&0.51&102.8&0.62&0.54&72.6\\
bar&1.62&0.58&97.6&1.73&0.98&29.1&
bar&0.50&0.21&118.1&0.55&0.22&50.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4448}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4450}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(r)a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4448.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4450.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.50&0.74&92.6&2.50&2.28&10.9&
R$^{\prime}$&3.43&2.20&164.1&3.56&3.04&145.7\\
r&1.47&0.49&92.2&1.51&1.47&82.6&
rs&1.51&0.96&10.0&1.64&1.28&44.2\\
&&&&&&&
bar&1.46&0.68&7.0&1.52&0.94&25.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4451}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4454}}}\\
\multicolumn{7}{c}{SA(r)0$^{+}$c }&
\multicolumn{7}{|c}{(RL)SAB(r)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4451.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4454.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.43&0.23&157.4&0.43&0.32&172.6&
RL&2.00&1.83&105.1&2.09&1.83&83.0\\
&&&&&&&
r&1.09&0.80&34.4&1.10&0.83&10.0\\
&&&&&&&
bar&1.02&0.49&22.0&1.02&0.51&175.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4457}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4460}}}\\
\multicolumn{7}{c}{(RR)SAB(l)0$^{+}$ }&
\multicolumn{7}{|c}{SA(r:)0$_{\rm c}$ sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4457.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4460.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&4.04&3.76&78.8&4.11&3.98&52.8&
r&0.42&0.13&38.9&0.49&0.42&95.4\\
R&2.42&2.24&162.7&2.61&2.24&93.3&
&&&&&&\\
bar&0.97&0.61&65.8&0.97&0.65&179.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4461}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4462}}}\\
\multicolumn{7}{c}{SA(r,l)0$^{+}$ }&
\multicolumn{7}{|c}{SAB$_{\rm x}$(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4461.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4462.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.47&0.54&5.1&1.58&1.34&134.2&
rs&1.33&0.41&118.6&1.33&0.90&174.8\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4491}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4492}}}\\
\multicolumn{7}{c}{SB(rs)0/a }&
\multicolumn{7}{|c}{SA(${\underline{\rm r}}$s)0$^{-}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4491.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4492.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.89&0.43&151.7&0.94&0.80&38.4&
${\underline{\rm r}}$s&0.48&0.42&55.9&0.50&0.45&55.0\\
bar&0.40&0.18&130.3&0.46&0.29&134.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4496A}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4498}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)d }&
\multicolumn{7}{|c}{SB(rs)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4496A.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4498.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.99&0.89&70.0&1.02&0.98&70.5&
rs&1.24&0.62&129.4&1.29&0.97&153.2\\
bar&0.53&0.11&52.6&0.53&0.12&168.7&
bar&1.05&0.19&123.5&1.10&0.30&155.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4501}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4504}}}\\
\multicolumn{7}{c}{SA(r${\underline{\rm s}}$)a${\underline{\rm b}}$ }&
\multicolumn{7}{|c}{SAB(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4501.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4504.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.55&0.61&137.4&1.59&1.18&159.9&
rs&0.93&0.71&134.1&1.18&0.92&98.6\\
&&&&&&&
bar&0.36&0.18&149.4&0.37&0.29&25.2\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4519}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4522}}}\\
\multicolumn{7}{c}{SAB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB$_{\rm a}$?(r,rs)a: pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4519.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4522.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.67&0.54&69.2&0.85&0.54&95.5&
R$^{\prime}$&2.38&0.56&32.9&2.41&2.12&158.6\\
bar&0.49&0.24&69.9&0.62&0.24&99.1&
r&1.32&0.36&35.4&1.39&1.28&57.7\\
&&&&&&&
rs&0.74&0.17&35.1&0.75&0.65&14.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4525}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4527}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)cd }&
\multicolumn{7}{|c}{(R$_{2}^{\prime}$)SAB(rs,nr)b${\underline{\rm c}}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4525.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4527.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.28&0.56&34.9&1.49&0.87&136.0&
R$_{2}^{\prime}$&4.75&0.95&65.4&4.79&3.41&169.1\\
bar&0.46&0.20&80.2&0.58&0.28&53.2&
rs&1.56&0.33&68.4&1.58&1.20&12.4\\
&&&&&&&
nr&0.23&0.07&61.7&0.28&0.20&120.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4528}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4531}}}\\
\multicolumn{7}{c}{SB(r)0$^{\rm o}$ }&
\multicolumn{7}{|c}{(L)SA(${\underline{\rm r}}$s)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4528.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4531.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.37&0.19&5.4&0.37&0.32&176.7&
${\underline{\rm r}}$s&0.69&0.46&164.8&0.74&0.64&51.1\\
bar&0.17&0.15&63.9&0.28&0.15&85.0&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4536}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4540}}}\\
\multicolumn{7}{c}{SAB(rs)${\underline{\rm b}}$c }&
\multicolumn{7}{|c}{SAB(rs)b: or SAB(rs)m /Sph, N }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4536.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4540.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&3.05&0.85&121.1&3.11&1.92&164.8&
rs&0.69&0.66&111.6&0.72&0.66&72.5\\
&&&&&&&
bar&0.30&0.12&53.6&0.30&0.13&177.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4548}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4565}}}\\
\multicolumn{7}{c}{SB(rs)a }&
\multicolumn{7}{|c}{SB$_{\rm x}$(r)${\underline{\rm a}}$b sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4548.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4565.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&2.04&1.52&85.2&2.56&1.56&103.7&
r&3.12&0.22&135.6&3.13&1.33&3.3\\
bar&1.93&0.90&61.3&2.49&0.90&91.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4567}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4568}}}\\
\multicolumn{7}{c}{SA(rs)bc }&
\multicolumn{7}{|c}{SA(r${\underline{\rm s}}$)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4567.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4568.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.51&0.37&36.6&0.71&0.41&106.7&
r${\underline{\rm s}}$&0.41&0.22&22.4&0.50&0.40&108.9\\
bar&0.28&0.21&56.0&0.36&0.25&109.9&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4569}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4579}}}\\
\multicolumn{7}{c}{(L)SB$_{\rm x}$(rs,x$_{1}$r)a }&
\multicolumn{7}{|c}{(RL,R$^{\prime}$)SB(r${\underline{\rm s}}$)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4569.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4579.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&4.01&1.76&17.5&4.73&3.66&121.4&
RL&4.33&3.10&96.7&4.39&4.10&27.5\\
x$_{1}$r&2.20&0.38&16.0&2.34&0.87&156.3&
R$^{\prime}$&3.13&2.20&98.7&3.18&2.90&29.6\\
&&&&&&&
r${\underline{\rm s}}$&2.22&1.34&66.1&2.44&1.62&135.4\\
&&&&&&&
bar&1.41&0.73&59.2&1.59&0.87&132.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4580}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4591}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(${\underline{\rm r}}$s$_{1}$,rs$_{2}$)a }&
\multicolumn{7}{|c}{SAB(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4580.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4591.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.86&1.26&161.6&1.88&1.64&20.8&
bar&0.28&0.10&38.7&0.28&0.19&6.2\\
${\underline{\rm r}}$s&1.12&0.81&158.3&1.12&1.06&19.4&
rs&0.26&0.15&31.1&0.30&0.26&115.2\\
rs&0.67&0.40&156.2&0.68&0.52&2.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4593}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4594}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(rs)a }&
\multicolumn{7}{|c}{(R)SA(l)0$^{+}$ sp/E1 }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4593.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4594.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&3.54&2.51&108.2&3.55&3.00&8.0&
R&4.59&0.44&89.0&4.59&1.06&0.4\\
rs&2.03&1.30&81.4&2.11&1.50&145.3&
&&&&&&\\
bar&1.75&0.70&57.5&1.95&0.75&126.2&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4596}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4597}}}\\
\multicolumn{7}{c}{(R${\underline{\rm L}}$)SB(rs)0/a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(s)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4596.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4597.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R{\underline{\rm L}}&3.40&2.66&140.1&3.63&3.07&49.1&
R$^{\prime}$&2.52&1.09&39.6&2.65&2.40&131.3\\
rs&2.11&1.44&82.3&2.34&1.60&126.7&
&&&&&&\\
bar&1.79&0.85&74.1&2.01&0.92&125.8&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4618}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4625}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(r${\underline{\rm s}}$)m }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(rs)m }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4618.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4625.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.26&2.03&33.2&2.78&2.22&81.0&
R$^{\prime}$&0.95&0.85&151.3&0.96&0.90&159.8\\
r${\underline{\rm s}}$&1.17&0.94&82.2&1.55&0.95&81.4&
rs&0.33&0.28&80.8&0.35&0.28&96.9\\
bar&0.68&0.25&65.3&0.83&0.27&61.8&
bar&0.27&0.17&23.2&0.28&0.18&46.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4628}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4639}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB$_{\rm a}$(s)a beams from ce }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(${\underline{\rm r}}$s)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4628.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4639.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.12&0.19&44.4&1.13&0.66&176.9&
R$^{\prime}$&2.36&1.38&116.4&2.63&1.90&134.2\\
&&&&&&&
${\underline{\rm r}}$s&0.89&0.79&127.6&1.22&0.89&92.5\\
&&&&&&&
bar&0.84&0.37&169.5&1.03&0.47&53.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4641}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4643}}}\\
\multicolumn{7}{c}{SA(rl)0$^{\rm o}$ }&
\multicolumn{7}{|c}{(L)SB(r,nl)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4641.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4643.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rl&0.19&0.17&35.4&0.20&0.18&119.4&
r&1.82&1.55&54.8&1.95&1.82&95.6\\
&&&&&&&
bar&1.59&0.84&132.3&1.96&0.85&79.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4647}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4651}}}\\
\multicolumn{7}{c}{SAB(rs)cd }&
\multicolumn{7}{|c}{SA(${\underline{\rm r}}$s)${\underline{\rm b}}$c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4647.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4651.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.27&0.17&12.2&0.35&0.18&74.3&
${\underline{\rm r}}$s&0.80&0.49&79.5&0.85&0.80&74.5\\
bar&0.14&0.09&114.1&0.14&0.11&147.0&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4654}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4658}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{SB(rs)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4654.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4658.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.17&0.73&126.8&1.36&1.14&71.3&
bar&0.31&0.08&36.0&0.41&0.11&52.8\\
bar&0.84&0.27&120.1&0.84&0.49&178.6&
rs&0.30&0.22&40.3&0.46&0.25&75.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4659}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4680}}}\\
\multicolumn{7}{c}{(R)SAB(l)0$^{\rm o}$ }&
\multicolumn{7}{|c}{SAB(rs)b /Sph }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4659.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4680.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.04&0.64&2.8&1.06&0.86&25.0&
rs&0.53&0.28&58.1&0.55&0.35&31.3\\
bar&0.26&0.22&72.4&0.36&0.22&86.1&
bar&0.31&0.12&168.5&0.37&0.13&121.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4682}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4689}}}\\
\multicolumn{7}{c}{SA(r)bc }&
\multicolumn{7}{|c}{(R)SA(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4682.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4689.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.22&0.16&82.6&0.32&0.22&90.9&
R&1.86&1.51&165.3&1.88&1.85&62.0\\
&&&&&&&
rs&0.57&0.44&127.2&0.64&0.48&120.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4691}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4698}}}\\
\multicolumn{7}{c}{(R$^{\prime}$L,R$^{\prime}$)SBm/S0/a }&
\multicolumn{7}{|c}{(R)SA(rr)0/a/E2 }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4691.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4698.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$L&2.79&2.15&25.3&2.81&2.59&161.7&
R&7.91&2.73&167.7&7.91&4.85&2.2\\
R$^{\prime}$&1.58&1.37&73.0&1.82&1.44&70.9&
r&2.15&0.71&169.4&2.15&1.25&6.3\\
bar&0.46&0.10&98.2&0.55&0.10&71.7&
r&1.58&0.50&168.9&1.58&0.89&5.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4699}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4710}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(l)0/a }&
\multicolumn{7}{|c}{SB$_{\rm x}$(nr)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4699.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4710.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.95&1.49&47.9&1.97&1.72&20.3&
nr&0.31&0.03&28.6&0.31&0.14&7.1\\
bar&0.41&0.22&48.5&0.42&0.26&13.2&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4713}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4722}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(rs)c }&
\multicolumn{7}{|c}{SB(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4713.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4722.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.44&0.38&65.0&0.61&0.42&98.6&
rs&0.65&0.18&30.5&0.65&0.48&167.1\\
bar&0.38&0.14&84.9&0.39&0.22&164.6&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4725}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4736}}}\\
\multicolumn{7}{c}{SAB(r,nb)a }&
\multicolumn{7}{|c}{(R)S${\underline{\rm A}}$B(rl,nr$^{\prime}$,nl,nb)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4725.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4736.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&4.35&1.37&48.8&4.53&1.93&23.5&
R&10.58&8.68&134.8&10.94&10.13&47.1\\
r&4.14&2.34&34.2&4.14&3.42&0.7&
bar&4.71&3.48&94.4&5.07&3.91&131.4\\
&&&&&&&
rl&4.48&3.47&103.9&4.70&3.99&136.6\\
&&&&&&&
nr$^{\prime}$&1.48&1.13&114.0&1.50&1.34&152.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4746}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4750}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)Sc sp }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(${\underline{\rm r}}$s)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4746.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4750.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.45&0.17&119.0&1.45&0.77&176.2&
R$^{\prime}$&1.52&1.33&156.7&1.69&1.51&101.5\\
&&&&&&&
${\underline{\rm r}}$s&0.55&0.49&146.0&0.63&0.53&103.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4771}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4772}}}\\
\multicolumn{7}{c}{SA(r)b sp }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(r)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4771.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4772.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.62&0.20&139.8&0.93&0.58&72.3&
R$^{\prime}$&3.85&1.93&147.4&3.86&3.68&19.5\\
&&&&&&&
r&2.36&0.61&145.3&2.36&1.16&178.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4779}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4791}}}\\
\multicolumn{7}{c}{SB(rs)b }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rl)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4779.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4791.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&0.95&0.29&9.2&1.13&0.31&114.2&
rl&0.32&0.18&55.7&0.33&0.25&155.8\\
rs&0.79&0.62&14.0&0.94&0.65&107.7&
bar&0.21&0.14&90.2&0.23&0.17&55.1\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4793}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4795}}}\\
\multicolumn{7}{c}{SA(rs)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(l)a pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4793.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4795.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.50&0.31&59.7&0.60&0.47&65.0&
R$^{\prime}$&1.38&1.13&116.5&1.56&1.38&87.1\\
&&&&&&&
bar&0.33&0.23&23.8&0.45&0.23&89.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4800}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4814}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(rs)a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(r${\underline{\rm s}}$)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4800.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4814.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.22&0.97&40.5&1.34&1.16&61.5&
R$^{\prime}$&1.45&0.85&117.8&1.47&1.08&159.3\\
rs&0.34&0.24&33.8&0.35&0.31&33.9&
r${\underline{\rm s}}$&0.84&0.58&112.0&0.89&0.72&141.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4818}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4826}}}\\
\multicolumn{7}{c}{(R)SB$_{\rm x}$(l)0$^{\rm o}$ }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(rs,r,nl)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4818.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4826.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&2.43&0.67&1.0&2.48&1.70&164.2&
R$^{\prime}$&7.17&3.10&117.1&7.18&5.59&4.5\\
&&&&&&&
rs&2.73&1.44&117.9&2.75&2.57&22.6\\
&&&&&&&
r&1.43&0.70&112.9&1.44&1.26&162.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4845}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4856}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB$_{\rm x}$(${\underline{\rm r}}$s,nd)0/a }&
\multicolumn{7}{|c}{(RL)SB0$^{-}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4845.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4856.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&4.35&0.87&82.0&4.47&3.30&19.9&
RL&2.44&0.65&36.2&2.46&1.79&169.3\\
${\underline{\rm r}}$s&2.09&0.34&76.2&2.17&1.29&159.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4866}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4880}}}\\
\multicolumn{7}{c}{(L)SA(rl)0$^{+}$ }&
\multicolumn{7}{|c}{(RL)S${\underline{\rm A}}$B(rl)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4866.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4880.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rl&2.52&0.31&87.0&2.53&1.29&175.4&
RL&2.05&1.48&148.0&2.13&1.80&143.2\\
&&&&&&&
rl&0.89&0.63&167.8&0.89&0.79&15.3\\
&&&&&&&
bar&0.29&0.18&169.0&0.30&0.22&11.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4897}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4900}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(${\underline{\rm r}}$s)b }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(s)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4897.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4900.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.48&0.31&164.9&0.48&0.37&21.2&
R$^{\prime}$&1.18&0.99&118.9&1.19&1.03&150.6\\
bar&0.40&0.20&5.7&0.43&0.23&42.1&
bar&0.72&0.23&140.1&0.72&0.24&179.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4902}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4941}}}\\
\multicolumn{7}{c}{SB(${\underline{\rm r}}$s)b }&
\multicolumn{7}{|c}{(RL)SA(${\underline{\rm r}}$s)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4902.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4941.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.88&0.79&171.9&0.95&0.79&78.0&
RL&3.33&2.36&22.5&3.33&3.09&175.5\\
bar&0.88&0.36&68.4&0.90&0.38&144.2&
${\underline{\rm r}}$s&1.96&0.96&20.0&1.97&1.25&174.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4951}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4961}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(rs)b }&
\multicolumn{7}{|c}{SB(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4951.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4961.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.67&0.64&90.8&1.89&1.67&95.8&
rs&0.40&0.26&105.3&0.41&0.36&25.1\\
rs&0.61&0.25&88.5&0.76&0.60&104.3&
bar&0.21&0.11&133.9&0.25&0.14&53.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4980}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4984}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(s)d /Sph }&
\multicolumn{7}{|c}{(R$^{\prime}$R)SAB$_{\rm a}$(l,nl)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4980.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4984.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.17&0.53&173.5&1.19&1.01&22.8&
R$^{\prime}$&5.07&2.82&24.7&5.07&4.77&0.5\\
bar&0.89&0.41&159.1&0.98&0.72&139.2&
R&3.26&1.90&20.1&3.39&3.10&136.6\\
&&&&&&&
bar&0.93&0.65&92.2&1.53&0.67&81.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4995}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5005}}}\\
\multicolumn{7}{c}{SAB$_{\rm a}$(rs)ab }&
\multicolumn{7}{|c}{(R$_{2}^{\prime}$)SAB$_{\rm x}$(${\underline{\rm r}}$s)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4995.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5005.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.72&0.63&118.6&1.01&0.69&82.4&
R$_{2}^{\prime}$&3.53&1.23&63.2&3.66&3.01&151.8\\
bar&0.64&0.31&34.5&0.93&0.33&107.1&
${\underline{\rm r}}$s&1.24&0.42&71.5&1.29&1.02&28.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5016}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5033}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(${\underline{\rm r}}$s)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5016.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5033.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.24&0.14&77.5&0.25&0.18&27.1&
R$^{\prime}$&8.84&4.26&167.0&9.07&7.75&153.3\\
bar&0.12&0.09&18.7&0.15&0.10&113.2&
rs&0.52&0.19&170.9&0.52&0.35&178.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5054}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5055}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(s,nr)bc }&
\multicolumn{7}{|c}{SA(rs,rl)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5054.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5055.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&4.45&2.48&157.6&4.45&4.06&6.7&
rs&1.40&0.64&93.8&1.45&1.10&152.6\\
nr&0.19&0.11&166.9&0.20&0.16&40.5&
rl&0.69&0.31&100.0&0.69&0.57&173.5\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5068}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5078}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)d }&
\multicolumn{7}{|c}{E(d)5/S(r)b sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5068.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5078.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&2.06&1.79&69.2&2.07&1.82&145.0&
r&0.71&0.09&146.0&0.71&0.27&177.5\\
bar&0.79&0.21&150.5&0.81&0.22&52.2&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5079}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5085}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(s)b }&
\multicolumn{7}{|c}{SA(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5079.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5085.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.68&0.42&25.2&0.82&0.68&100.4&
rs&0.28&0.19&45.8&0.28&0.21&171.6\\
bar&0.36&0.16&157.6&0.61&0.19&108.2&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5088}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5101}}}\\
\multicolumn{7}{c}{(R)SA${\underline{\rm B}}$d }&
\multicolumn{7}{|c}{(R$_{1}$R$_{2}^{\prime}$)SB(${\underline{\rm r}}$s,nl?)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5088.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5101.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.43&0.41&177.2&1.44&1.17&164.9&
R$_{2}^{\prime}$&5.31&4.61&153.9&5.46&4.84&45.4\\
&&&&&&&
R$_{1}$&4.24&3.37&3.8&4.50&3.42&66.1\\
&&&&&&&
${\underline{\rm r}}$s&1.70&1.41&122.3&1.70&1.52&175.6\\
&&&&&&&
bar&1.62&0.76&122.0&1.62&0.82&176.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5105}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5112}}}\\
\multicolumn{7}{c}{SAB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5105.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5112.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.54&0.42&134.8&0.57&0.54&93.6&
r${\underline{\rm s}}$&1.37&0.59&118.5&1.37&0.88&177.5\\
bar&0.19&0.10&1.4&0.23&0.11&60.4&
bar&0.33&0.05&131.5&0.33&0.08&18.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5117}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5122}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(s)d }&
\multicolumn{7}{|c}{S0$^{-}$ sp + PR sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5117.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5122.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.08&0.69&160.6&1.31&1.05&73.1&
PRG&1.79&0.16&25.6&$-$&$-$&$-$\\
bar&0.78&0.24&157.5&0.79&0.44&12.0&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5134}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5145}}}\\
\multicolumn{7}{c}{(R)SA${\underline{\rm B}}$(rs)0/a }&
\multicolumn{7}{|c}{SA(r,nl)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5134.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5145.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&3.53&2.99&71.8&3.53&3.09&171.0&
r&0.34&0.18&86.5&0.34&0.23&21.1\\
bar&1.55&0.60&154.7&1.60&0.60&76.3&
&&&&&&\\
rs&1.51&0.74&150.2&1.56&0.74&72.1&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5147}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5170}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB$_{\rm x,box}$(l)0/a sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5147.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5170.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.10&0.96&128.3&1.19&1.09&77.2&
R$^{\prime}$&4.85&0.29&126.0&4.85&1.97&177.9\\
bar&0.35&0.18&12.0&0.42&0.18&76.8&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5194}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5195}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(rs,nr$^{\prime}$)bc }&
\multicolumn{7}{|c}{SAB(r)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5194.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5195.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.84&0.75&87.0&0.97&0.77&73.4&
r&1.54&1.41&130.5&1.91&1.51&81.7\\
bar&0.74&0.50&138.4&0.88&0.50&96.3&
bar&1.34&0.84&177.8&1.74&0.85&80.1\\
nr$^{\prime}$&0.44&0.41&79.8&0.50&0.42&77.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5205}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5218}}}\\
\multicolumn{7}{c}{SB(rs)ab }&
\multicolumn{7}{|c}{SB(rs)a pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5205.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5218.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.55&0.38&167.0&0.70&0.55&89.5&
rs&0.63&0.35&69.3&0.72&0.36&114.2\\
bar&0.37&0.19&107.5&0.63&0.21&103.9&
bar&0.45&0.17&97.9&0.48&0.19&143.6\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5236}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5247}}}\\
\multicolumn{7}{c}{SAB(s,nr)c }&
\multicolumn{7}{|c}{SA(r)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5236.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5247.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&4.18&1.29&53.7&4.33&1.32&51.5&
r&0.30&0.25&5.3&0.34&0.26&108.8\\
nr&0.33&0.20&158.5&0.33&0.21&151.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5248}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5289}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(s,nr)b${\underline{\rm c}}$ }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(rl)0/a sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5248.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5289.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&5.97&4.36&100.2&5.99&5.55&163.7&
R$^{\prime}$&1.31&0.24&97.7&1.32&0.90&168.2\\
bar&2.81&1.17&125.2&2.94&1.44&29.5&
rl&0.42&0.09&98.8&0.42&0.36&170.8\\
nr&0.22&0.19&139.5&0.26&0.20&68.9&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5300}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5313}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(r${\underline{\rm s}}$)c }&
\multicolumn{7}{|c}{SA(r)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5300.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5313.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.55&0.32&133.6&0.61&0.45&135.7&
r&0.42&0.24&49.8&0.43&0.40&38.1\\
bar&0.30&0.18&163.9&0.33&0.26&47.7&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5320}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5334}}}\\
\multicolumn{7}{c}{SA(r$^{\prime}$l)bc }&
\multicolumn{7}{|c}{SB(rs,x$_{1}$r)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5320.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5334.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r$^{\prime}$l&0.23&0.15&20.7&0.31&0.23&85.1&
rs&0.84&0.78&118.3&1.10&0.78&92.7\\
&&&&&&&
bar&0.44&0.15&47.1&0.48&0.17&41.7\\
&&&&&&&
x$_{1}$r&0.42&0.11&44.7&0.45&0.14&38.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5336}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5337}}}\\
\multicolumn{7}{c}{SAB(rs)c }&
\multicolumn{7}{|c}{SB(rs)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5336.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5337.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.23&0.17&44.5&0.28&0.18&109.4&
rs&0.41&0.22&18.3&0.48&0.40&104.3\\
bar&0.20&0.12&78.9&0.21&0.14&145.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5338}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5339}}}\\
\multicolumn{7}{c}{SB(${\underline{\rm r}}$s)0$^{\rm o}$ }&
\multicolumn{7}{|c}{SB(rs)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5338.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5339.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.48&0.30&90.8&0.62&0.48&95.1&
rs&0.92&0.76&22.2&1.05&0.86&113.3\\
&&&&&&&
bar&0.79&0.23&81.8&0.87&0.27&42.2\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5347}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5350}}}\\
\multicolumn{7}{c}{SB(${\underline{\rm r}}$s)a }&
\multicolumn{7}{|c}{SB(${\underline{\rm r}}$s)a${\underline{\rm b}}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5347.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5350.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&1.01&0.42&100.9&1.01&0.45&12.8&
${\underline{\rm r}}$s&0.80&0.53&42.6&0.83&0.80&100.6\\
${\underline{\rm r}}$s&1.00&0.73&105.7&1.01&0.78&21.4&
bar&0.73&0.29&122.1&1.13&0.29&83.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5364}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5371}}}\\
\multicolumn{7}{c}{SA(r,is)b }&
\multicolumn{7}{|c}{SAB(r${\underline{\rm s}}$)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5364.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5371.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.15&0.66&40.2&1.16&0.98&16.2&
r${\underline{\rm s}}$&0.82&0.62&42.2&0.90&0.71&51.6\\
&&&&&&&
bar&0.70&0.42&99.8&0.88&0.42&86.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5375}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5376}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB$_{\rm a}$(${\underline{\rm r}}$s,bl)a }&
\multicolumn{7}{|c}{SA(${\underline{\rm r}}$s,l)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5375.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5376.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.24&1.82&164.7&2.25&2.09&16.0&
${\underline{\rm r}}$s&0.57&0.38&57.8&0.66&0.56&106.2\\
bar&0.91&0.38&168.0&0.91&0.44&10.7&
&&&&&&\\
${\underline{\rm r}}$s&0.85&0.75&7.0&0.91&0.81&61.4&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5377}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5383}}}\\
\multicolumn{7}{c}{(R$_{1}$)SA${\underline{\rm B}}$(s,nl)0/a }&
\multicolumn{7}{|c}{SB(rs,nr)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5377.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5383.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{1}$&4.05&2.03&21.4&4.19&3.64&146.7&
rs&1.98&1.72&102.4&2.11&1.96&106.2\\
bar&3.17&1.11&44.3&3.62&1.81&39.0&
bar&1.67&0.61&123.5&1.69&0.73&16.6\\
&&&&&&&
nr&0.29&0.14&79.1&0.31&0.16&139.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5426}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5427}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(rs)c }&
\multicolumn{7}{|c}{SA(r)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5426.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5427.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.66&0.31&4.2&0.78&0.53&49.8&
r&0.22&0.15&29.3&0.24&0.16&130.2\\
bar&0.17&0.10&177.2&0.20&0.16&69.8&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5430}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5443}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s,tb)b }&
\multicolumn{7}{|c}{(R$^{\prime}$L)SAB$_{\rm x}$(${\underline{\rm r}}$s)a sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5430.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5443.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.59&0.83&12.1&1.63&1.23&22.0&
R$^{\prime}$L&2.50&0.73&36.9&2.52&1.94&10.8\\
bar&0.56&0.23&153.6&0.65&0.29&133.2&
${\underline{\rm r}}$s&1.38&0.36&34.3&1.38&0.96&176.2\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5448}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5457}}}\\
\multicolumn{7}{c}{(R$_{1}$)SAB(${\underline{\rm r}}$s)a }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(r${\underline{\rm s}}$)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5448.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5457.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{1}$&3.34&1.34&115.7&3.62&2.96&43.3&
r${\underline{\rm s}}$&1.81&1.60&178.7&1.88&1.65&124.1\\
${\underline{\rm r}}$s&1.67&0.54&110.2&1.67&1.28&179.9&
bar&0.84&0.58&80.4&0.87&0.60&48.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5472}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5492}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB$_{\rm a}$0/a }&
\multicolumn{7}{|c}{SA(rs)b: sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5472.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5492.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.59&0.17&35.0&0.59&0.45&172.4&
rs&0.40&0.09&150.0&0.40&0.33&18.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5523}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5534}}}\\
\multicolumn{7}{c}{SA(rs)cd }&
\multicolumn{7}{|c}{(R$^{\prime}$L)SB(r${\underline{\rm s}}$)a pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5523.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5534.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.81&0.22&89.8&0.89&0.72&135.6&
R$^{\prime}$L&1.21&0.83&170.3&1.30&0.86&58.7\\
&&&&&&&
r${\underline{\rm s}}$&0.50&0.37&77.6&0.53&0.39&127.2\\
&&&&&&&
bar&0.50&0.22&74.9&0.53&0.23&130.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5566}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5577}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(r,nr$^{\prime}$)a }&
\multicolumn{7}{|c}{SA(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5566.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5577.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&5.07&1.47&36.0&5.09&3.99&7.4&
rs&0.40&0.16&62.3&0.60&0.37&72.2\\
r&1.35&0.74&24.8&2.10&1.28&102.6&
&&&&&&\\
nr$^{\prime}$&0.20&0.08&34.1&0.22&0.20&100.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5584}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5587}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{SA(r)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5584.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5587.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.31&0.27&27.4&0.42&0.29&80.0&
r&0.64&0.16&158.2&0.67&0.45&157.0\\
bar&0.27&0.14&35.9&0.36&0.15&70.1&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5595}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5600}}}\\
\multicolumn{7}{c}{SAB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{SB(rs)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5595.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5600.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.36&0.31&53.0&0.51&0.36&87.9&
bar&0.44&0.20&155.6&0.45&0.21&166.1\\
&&&&&&&
rs&0.44&0.35&144.0&0.45&0.37&147.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5602}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5633}}}\\
\multicolumn{7}{c}{(RL)SA(l)0$^{+}$ }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(r)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5602.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5633.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&1.05&0.54&166.2&1.05&0.97&165.1&
r&0.46&0.30&10.3&0.46&0.39&157.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5636}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5665}}}\\
\multicolumn{7}{c}{SAB(r)0/a }&
\multicolumn{7}{|c}{SAB(rs)c pec /Sph }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5636.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5665.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.84&0.52&35.3&0.85&0.56&152.1&
rs&0.95&0.60&139.8&1.09&0.85&123.9\\
bar&0.68&0.23&76.3&0.68&0.26&20.6&
bar&0.20&0.09&128.9&0.24&0.12&133.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5668}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5669}}}\\
\multicolumn{7}{c}{SAB(rs)cd }&
\multicolumn{7}{|c}{SB(rs)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5668.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5669.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.41&0.37&146.7&0.43&0.41&79.8&
rs&0.38&0.31&89.1&0.45&0.35&70.5\\
bar&0.38&0.25&106.5&0.41&0.27&134.3&
bar&0.17&0.04&40.5&0.17&0.05&152.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5678}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5689}}}\\
\multicolumn{7}{c}{(R$^{\prime}$:)SA(${\underline{\rm r}}$s)b /RG }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB$_{\rm boxy}$(rl,nd)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5678.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5689.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.31&1.17&1.3&2.32&2.14&169.1&
R$^{\prime}$&2.50&0.40&83.9&2.50&1.49&179.1\\
${\underline{\rm r}}$s&1.35&0.57&178.3&1.36&1.03&164.9&
rl&1.05&0.25&87.0&1.10&0.88&31.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5690}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5701}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)d sp }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$)SB(rl)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5690.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5701.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.03&0.39&141.6&2.03&1.60&177.2&
R$_{1}^{\prime}$&3.21&2.72&77.2&3.24&2.80&32.7\\
&&&&&&&
rl&1.34&1.08&178.3&1.37&1.10&123.6\\
&&&&&&&
bar&1.28&0.74&177.2&1.31&0.75&125.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5713}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5719}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(rs)ab: pec }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(nr)0/a sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5713.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5719.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.67&1.48&87.2&1.89&1.49&82.1&
R$^{\prime}$&1.42&0.35&104.2&1.47&0.97&20.7\\
rs&0.65&0.49&88.8&0.73&0.49&79.8&
nr&0.17&0.05&100.3&0.17&0.15&7.0\\
bar&0.39&0.14&95.7&0.44&0.14&83.1&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5728}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5740}}}\\
\multicolumn{7}{c}{(R$_{1}$)SB(${\underline{\rm r}}$s,nr,nb)0/a }&
\multicolumn{7}{|c}{(R)SA${\underline{\rm B}}$(r)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5728.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5740.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{1}$&3.61&2.34&1.3&3.65&3.17&161.9&
R&2.16&1.17&156.3&2.34&2.04&127.3\\
bar&1.89&0.57&33.4&2.06&0.72&36.5&
r&0.70&0.41&157.3&0.80&0.68&108.0\\
${\underline{\rm r}}$s&1.81&0.89&33.0&1.99&1.11&40.8&
bar&0.53&0.28&127.8&0.78&0.36&115.3\\
nr&0.20&0.12&7.9&0.20&0.16&3.1&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5744}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5746}}}\\
\multicolumn{7}{c}{SAB(rs)ab: pec }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB$_{\rm x}$(r,nd)0/a sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5744.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5746.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.27&0.18&132.9&0.29&0.23&43.8&
R$^{\prime}$&5.06&0.39&170.7&5.09&2.02&6.8\\
&&&&&&&
r&2.43&0.25&171.4&2.47&1.28&12.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5750}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5756}}}\\
\multicolumn{7}{c}{(RL)SAB(rr)0/a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA${\underline{\rm B}}$(s)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5750.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5756.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&2.70&1.30&66.6&2.80&2.52&39.3&
R$^{\prime}$&2.80&1.02&63.9&2.90&2.37&26.9\\
r&1.56&0.80&63.2&1.61&1.56&81.1&
&&&&&&\\
r&1.13&0.56&63.4&1.14&1.12&44.0&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5757}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5768}}}\\
\multicolumn{7}{c}{(R$_{2}^{\prime}$)SB(rs)${\underline{\rm a}}$b }&
\multicolumn{7}{|c}{SAB(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5757.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5768.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{2}^{\prime}$&1.35&1.19&50.7&1.46&1.31&67.2&
rs&0.55&0.50&113.8&0.55&0.54&152.8\\
rs&0.77&0.53&161.2&0.87&0.56&118.4&
bar&0.36&0.16&149.2&0.37&0.17&31.4\\
bar&0.66&0.23&164.8&0.73&0.25&127.8&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5770}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5777}}}\\
\multicolumn{7}{c}{SAB(r,bl)0$^{+}$ }&
\multicolumn{7}{|c}{(R)SB$_{\rm box}$(l,nl)0$^{+}$ sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5770.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5777.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.75&0.72&71.4&0.79&0.73&74.8&
R&2.08&0.17&142.8&2.08&0.79&177.5\\
bar&0.73&0.41&111.5&0.79&0.42&75.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5781}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5792}}}\\
\multicolumn{7}{c}{(R)SB(rs)a/d }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$)SAB(r,nd,nr)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5781.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5792.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.36&0.78&28.5&1.59&1.31&111.4&
R$_{1}^{\prime}$&7.09&1.19&81.6&7.55&3.38&156.3\\
rs&0.72&0.43&28.6&0.86&0.70&107.8&
r&2.35&0.69&85.6&2.42&2.02&154.2\\
bar&0.25&0.05&30.0&0.25&0.09&169.2&
nr&0.18&0.06&84.1&0.20&0.16&139.0\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5806}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5809}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(rs,nr)ab }&
\multicolumn{7}{|c}{SA(rs)a /Sph }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5806.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5809.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.68&1.46&170.1&2.77&2.56&42.5&
rs&0.37&0.12&147.2&0.37&0.28&177.6\\
bar&1.25&0.40&176.3&1.30&0.70&22.2&
&&&&&&\\
rs&1.23&0.76&175.7&1.44&1.17&65.5&
&&&&&&\\
nr&0.12&0.07&162.5&0.14&0.12&107.7&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5821}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5850}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(r)a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(r,nr,nb)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5821.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5850.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.53&0.31&145.6&0.54&0.52&166.7&
R$^{\prime}$&4.00&3.31&3.8&4.26&3.84&58.6\\
bar&0.17&0.10&144.0&0.18&0.17&114.9&
bar&2.09&0.79&116.7&2.42&0.85&120.0\\
&&&&&&&
r&2.09&1.83&122.8&2.47&1.91&105.5\\
&&&&&&&
nr&0.26&0.22&150.6&0.28&0.25&122.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5854}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5878}}}\\
\multicolumn{7}{c}{(R)SB$_{\rm x}$(r)0$^{+}$ }&
\multicolumn{7}{|c}{SAB$_{\rm ax}$(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5854.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5878.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.67&0.39&50.5&1.73&1.15&158.9&
rs&1.08&0.39&10.3&1.23&0.93&48.0\\
r&0.66&0.18&57.4&0.68&0.53&22.4&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5879}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5892}}}\\
\multicolumn{7}{c}{SAB$_{\rm a}$(rs)bc }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5879.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5892.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.58&0.27&5.0&0.71&0.58&85.6&
r${\underline{\rm s}}$&0.45&0.39&144.1&0.48&0.41&62.0\\
&&&&&&&
bar&0.16&0.09&157.1&0.17&0.09&56.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5899}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5900}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)bc }&
\multicolumn{7}{|c}{(R$^{\prime}$)Sb sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5899.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5900.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.49&0.32&5.4&0.86&0.47&99.4&
R$^{\prime}$&1.15&0.09&127.7&1.15&0.40&179.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5913}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5915}}}\\
\multicolumn{7}{c}{(RL)SB(r)0/a }&
\multicolumn{7}{|c}{SA(r:)c: pec }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5913.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5915.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&2.29&0.84&159.5&2.30&1.92&170.6&
r&0.42&0.30&80.8&0.55&0.31&76.9\\
r&0.98&0.45&163.6&1.05&0.96&59.9&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5921}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5930}}}\\
\multicolumn{7}{c}{SB(${\underline{\rm r}}$s)b }&
\multicolumn{7}{|c}{(L)SAB$_{\rm a}$(rs)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5921.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5930.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&1.52&0.44&18.6&1.72&0.47&59.6&
rs&0.42&0.26&159.4&0.50&0.41&97.1\\
${\underline{\rm r}}$s&1.19&0.82&23.7&1.38&0.85&69.3&
bar&0.25&0.18&73.2&0.46&0.18&90.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5937}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5953}}}\\
\multicolumn{7}{c}{SA(rs)bc }&
\multicolumn{7}{|c}{SA(r)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5937.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5953.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.22&0.17&40.8&0.30&0.20&77.9&
r&0.21&0.17&72.9&0.22&0.18&47.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5954}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5956}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(rs)b }&
\multicolumn{7}{|c}{SB(${\underline{\rm r}}$s)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5954.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5956.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.70&0.28&178.8&0.71&0.44&167.2&
${\underline{\rm r}}$s&0.27&0.23&15.4&0.28&0.23&103.9\\
rs&0.28&0.17&0.2&0.29&0.27&146.5&
bar&0.23&0.13&30.7&0.23&0.13&120.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~5957}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5958}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(${\underline{\rm r}}$s,bl)a }&
\multicolumn{7}{|c}{SB(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5957.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5958.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.38&2.08&165.4&2.43&2.25&138.2&
rs&0.38&0.34&176.7&0.39&0.37&125.1\\
bar&0.96&0.41&95.1&1.06&0.41&92.0&
bar&0.19&0.09&137.5&0.20&0.10&124.6\\
${\underline{\rm r}}$s&0.94&0.92&118.7&1.04&0.93&93.8&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~5962}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~5964}}}\\
\multicolumn{7}{c}{SAB(rs,nr)c }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5962.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC5964.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.65&0.31&109.1&0.65&0.43&5.7&
r${\underline{\rm s}}$&1.17&0.86&121.3&1.37&1.01&119.5\\
bar&0.39&0.19&147.7&0.47&0.22&57.3&
bar&0.60&0.09&147.7&0.60&0.12&176.2\\
nr&0.13&0.08&81.5&0.15&0.11&130.9&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~6012}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~6014}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(r,x$_{1}$r)ab }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(rs,bl)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6012.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6014.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.57&2.32&168.5&2.91&2.44&106.6&
bar&0.56&0.36&31.2&0.66&0.37&70.2\\
r&1.48&0.94&166.7&1.61&1.03&130.0&
rs&0.54&0.52&111.9&0.65&0.53&96.8\\
x$_{1}$r&0.74&0.15&151.7&0.84&0.16&121.7&
&&&&&&\\
bar&0.63&0.17&156.1&0.70&0.19&125.6&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~6070}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~6155}}}\\
\multicolumn{7}{c}{SA(r)c }&
\multicolumn{7}{|c}{(R$^{\prime}$R$^{\prime}$)SB(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6070.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6155.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.08&0.44&60.6&1.09&0.95&7.3&
R$^{\prime}$&1.08&0.70&145.0&1.09&0.93&17.6\\
&&&&&&&
R$^{\prime}$&0.52&0.40&147.8&0.55&0.50&57.8\\
&&&&&&&
rs&0.23&0.20&14.6&0.29&0.20&79.1\\
&&&&&&&
bar&0.19&0.10&120.7&0.20&0.13&147.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~6207}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~6217}}}\\
\multicolumn{7}{c}{SAB(rs)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(rs)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6207.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6217.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.62&0.26&2.6&0.69&0.40&140.8&
R$^{\prime}$&2.72&2.46&91.1&2.73&2.68&164.8\\
bar&0.27&0.12&36.6&0.30&0.19&42.6&
rs&1.34&1.00&158.0&1.44&1.02&70.3\\
&&&&&&&
bar&1.23&0.33&149.3&1.30&0.33&58.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~6267}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~6278}}}\\
\multicolumn{7}{c}{SB(rs)b }&
\multicolumn{7}{|c}{(L)SA(r)0$^{\rm o}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6267.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6278.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.70&0.53&53.1&0.79&0.68&64.3&
r&0.43&0.20&115.9&0.45&0.32&146.5\\
bar&0.57&0.15&157.6&0.77&0.16&108.5&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~6340}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~6412}}}\\
\multicolumn{7}{c}{(R)SA(l)0/a }&
\multicolumn{7}{|c}{SB(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6340.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6412.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.80&1.52&98.8&2.02&1.54&103.5&
rs&0.42&0.33&69.7&0.44&0.33&72.4\\
&&&&&&&
bar&0.25&0.14&160.9&0.25&0.15&157.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~6434}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~6870}}}\\
\multicolumn{7}{c}{(R)SAB$_{\rm a}$(rs)b }&
\multicolumn{7}{|c}{SAB(r$^{\prime}$r$^{\prime}$)a + PR? }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6434.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6870.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.25&0.50&92.6&1.27&1.11&161.5&
PRG&1.89&1.40&102.0&$-$&$-$&$-$\\
rs&0.50&0.25&88.2&0.60&0.48&114.8&
rs&1.17&0.39&87.1&1.19&1.01&20.1\\
&&&&&&&
rs&0.78&0.23&85.7&0.78&0.60&6.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~6887}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~6889}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)b }&
\multicolumn{7}{|c}{SB(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6887.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6889.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.52&0.19&106.5&0.54&0.51&56.1&
rs&0.26&0.19&71.7&0.27&0.26&122.7\\
&&&&&&&
bar&0.17&0.10&163.5&0.23&0.10&90.5\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~6902}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~6923}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(${\underline{\rm r}}$s,nl)a }&
\multicolumn{7}{|c}{SAB$_{\rm a}$(rl)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6902.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6923.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.68&0.58&147.8&0.71&0.68&91.6&
rl&0.36&0.17&73.4&0.36&0.25&178.9\\
bar&0.60&0.34&129.4&0.62&0.41&151.3&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~6925}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7051}}}\\
\multicolumn{7}{c}{SB(rs)b }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$R$_{2}^{\prime}$)SAB$_{\rm a}$(rs)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC6925.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7051.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.97&0.25&6.0&0.97&0.76&172.9&
R$_{2}^{\prime}$&1.12&0.97&57.4&1.13&1.04&163.5\\
&&&&&&&
R$_{1}^{\prime}$&0.76&0.58&179.4&0.81&0.59&108.4\\
&&&&&&&
rs&0.29&0.22&78.4&0.30&0.23&15.7\\
&&&&&&&
bar&0.28&0.14&79.4&0.28&0.15&14.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7070}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7098}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)c }&
\multicolumn{7}{|c}{(R)SAB$_{\rm a}$(r$^{\prime}$l,nl,nb)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7070.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7098.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.38&0.28&170.4&0.40&0.30&140.8&
R&3.63&2.26&80.7&4.13&3.46&62.9\\
bar&0.23&0.12&77.6&0.26&0.12&64.7&
r$^{\prime}$l&1.87&1.07&67.8&1.95&1.78&134.9\\
&&&&&&&
bar&1.38&0.63&50.6&1.63&0.93&133.1\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~7107}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7140}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(r${\underline{\rm s}}$)dm }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA${\underline{\rm B}}$$_{\rm x}$(rs,nl)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7107.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7140.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.33&1.06&121.4&1.38&1.18&38.2&
R$^{\prime}$&3.72&2.60&176.0&4.13&3.62&113.2\\
r${\underline{\rm s}}$&0.82&0.60&120.2&0.84&0.66&30.3&
rs&1.94&1.16&22.0&2.19&1.59&48.6\\
bar&0.50&0.16&130.4&0.52&0.18&34.1&
bar&1.92&0.48&19.1&2.02&0.71&25.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7162}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7179}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SAB(rs)c }&
\multicolumn{7}{|c}{SB$_{\rm xa}$(r)0/a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7162.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7179.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.19&0.47&11.4&1.20&1.11&159.9&
bar&0.91&0.23&44.7&0.93&0.44&166.6\\
rs&0.38&0.22&13.7&0.52&0.38&88.1&
r&0.89&0.41&50.4&0.89&0.80&179.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7184}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7188}}}\\
\multicolumn{7}{c}{SB(r,nd)ab }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(s)b: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7184.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7188.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.71&0.42&59.1&1.71&1.64&164.6&
R$^{\prime}$&0.79&0.37&48.6&0.80&0.74&28.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~7191}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7205}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA${\underline{\rm B}}$(s)b pec }&
\multicolumn{7}{|c}{SA(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7191.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7205.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.83&0.37&133.5&0.90&0.80&122.4&
rs&0.47&0.25&63.1&0.52&0.46&115.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7213}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7218}}}\\
\multicolumn{7}{c}{(L)SA(r,l)0$^{\rm o}$ }&
\multicolumn{7}{|c}{SB(rs)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7213.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7218.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.88&0.79&5.2&0.90&0.82&42.9&
rs&0.54&0.37&28.2&0.82&0.53&83.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7219}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7290}}}\\
\multicolumn{7}{c}{(R$_{2}^{\prime}$)S${\underline{\rm A}}$B(r)a }&
\multicolumn{7}{|c}{SA(rs)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7219.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7290.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{2}^{\prime}$&1.36&0.83&33.0&1.39&1.27&31.6&
rs&0.36&0.21&156.7&0.38&0.36&105.4\\
r&0.33&0.24&50.3&0.41&0.30&67.2&
&&&&&&\\
bar&0.29&0.20&86.7&0.42&0.21&76.9&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~7314}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7328}}}\\
\multicolumn{7}{c}{SAB(rs)bc }&
\multicolumn{7}{|c}{SAB(rs)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7314.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7328.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.08&0.32&179.6&1.10&0.80&164.5&
rs&0.36&0.23&65.3&0.61&0.32&103.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7378}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7416}}}\\
\multicolumn{7}{c}{(L)SA(${\underline{\rm r}}$s)0/a }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(r)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7378.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7416.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.64&0.26&0.8&0.65&0.42&10.9&
R$^{\prime}$&2.74&0.43&108.9&2.74&1.65&0.8\\
&&&&&&&
r&1.25&0.29&109.2&1.25&1.10&6.8\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7418}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7421}}}\\
\multicolumn{7}{c}{SAB(rs)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(rs,bl)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7418.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7421.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&1.10&0.25&119.5&1.12&0.33&163.5&
R$^{\prime}$&1.68&1.54&76.7&1.76&1.66&71.8\\
rs&1.07&0.71&107.1&1.18&0.87&131.1&
rs&0.91&0.74&75.1&0.92&0.83&23.5\\
&&&&&&&
bar&0.73&0.25&93.0&0.76&0.28&32.3\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~7424}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7437}}}\\
\multicolumn{7}{c}{SB$_{\rm a}$(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rs)c: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7424.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7437.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.27&0.90&71.5&1.34&0.94&50.8&
rs&0.42&0.32&70.0&0.45&0.34&58.5\\
bar&0.36&0.11&133.3&0.39&0.11&102.4&
bar&0.24&0.16&13.9&0.24&0.18&164.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7463}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7465}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)c }&
\multicolumn{7}{|c}{E(d)1-2?/S0$^{-}$ sp + PR material?}\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7463.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7465.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.38&0.18&75.2&0.54&0.31&116.7&
PRG&0.71&0.09&160.1&$-$&$-$&$-$\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7479}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7496}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)b }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7479.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7496.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&2.77&2.13&27.6&2.92&2.69&57.2&
r${\underline{\rm s}}$&1.43&1.00&160.2&1.47&1.02&123.7\\
bar&1.65&0.41&8.1&1.68&0.53&164.3&
bar&1.33&0.31&147.9&1.37&0.32&113.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~7513}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7531}}}\\
\multicolumn{7}{c}{SB(rs)a }&
\multicolumn{7}{|c}{SAB$_{\rm x}$(r)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7513.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7531.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.31&0.87&90.2&1.46&1.17&127.5&
bar&0.99&0.33&11.7&1.03&0.59&156.3\\
bar&1.27&0.34&71.0&1.51&0.43&131.9&
r&0.95&0.39&17.1&0.96&0.72&164.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7537}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7552}}}\\
\multicolumn{7}{c}{SA(${\underline{\rm r}}$s)c }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$)SB(r${\underline{\rm s}}$,nr)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7537.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7552.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.24&0.11&76.9&0.34&0.24&90.5&
R$_{1}^{\prime}$&3.08&2.52&179.1&3.14&2.57&135.0\\
&&&&&&&
r${\underline{\rm s}}$&1.96&1.23&99.7&2.02&1.24&63.3\\
&&&&&&&
bar&1.20&0.43&91.2&1.23&0.44&54.1\\
&&&&&&&
nr&0.12&0.10&104.7&0.12&0.10&71.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7582}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7590}}}\\
\multicolumn{7}{c}{(R$_{1}^{\prime}$)SB(r${\underline{\rm s}}$)a }&
\multicolumn{7}{|c}{SAB(r${\underline{\rm s}}$)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7582.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7590.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{1}^{\prime}$&4.03&1.77&148.5&4.12&3.75&148.5&
r${\underline{\rm s}}$&0.85&0.31&33.8&0.88&0.82&41.3\\
r${\underline{\rm s}}$&1.97&0.79&154.2&2.00&1.69&20.7&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~7606}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7689}}}\\
\multicolumn{7}{c}{SA(r)b }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rs)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7606.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7689.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.85&0.38&140.2&1.02&0.81&113.4&
bar&0.26&0.10&100.8&0.30&0.13&136.5\\
&&&&&&&
rs&0.26&0.22&134.5&0.33&0.26&85.9\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7690}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7716}}}\\
\multicolumn{7}{c}{SA(r)0/a }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(r)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7690.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7716.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.23&0.11&128.1&0.23&0.22&171.0&
r&0.47&0.34&30.3&0.47&0.40&178.0\\
&&&&&&&
bar&0.13&0.10&54.3&0.14&0.11&39.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7723}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7724}}}\\
\multicolumn{7}{c}{SB(rs)ab }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(${\underline{\rm r}}$s)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7723.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7724.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.71&0.55&54.0&0.85&0.69&73.6&
R$^{\prime}$&0.88&0.54&33.4&0.88&0.78&14.1\\
bar&0.64&0.23&68.4&0.73&0.30&42.8&
bar&0.36&0.17&62.6&0.42&0.21&49.5\\
&&&&&&&
${\underline{\rm r}}$s&0.30&0.20&77.1&0.39&0.22&67.8\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~7731}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7741}}}\\
\multicolumn{7}{c}{(R$_{1}$R$_{2}^{\prime}$)S${\underline{\rm A}}$B(r)a }&
\multicolumn{7}{|c}{(R$_{2}^{\prime}$)SB(s)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7731.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7741.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{2}^{\prime}$&1.09&0.85&92.6&1.27&1.03&66.9&
R$_{2}^{\prime}$&2.76&2.23&168.8&3.21&2.74&79.2\\
R$_{1}$&0.69&0.53&88.9&0.78&0.66&64.4&
bar&1.46&0.49&95.9&2.00&0.52&107.0\\
bar&0.28&0.15&43.3&0.32&0.19&131.1&
&&&&&&\\
r&0.27&0.22&50.5&0.33&0.26&107.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7742}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7743}}}\\
\multicolumn{7}{c}{SA(rr)0$^{+}$ }&
\multicolumn{7}{|c}{SAB(${\underline{\rm r}}$s)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7742.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7743.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.73&0.68&119.8&0.74&0.70&54.2&
${\underline{\rm r}}$s&1.38&1.14&119.4&1.80&1.16&79.6\\
r&0.34&0.32&142.3&0.35&0.32&67.6&
bar&1.32&0.63&94.7&1.52&0.73&51.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~7750}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~7755}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(rs)bc }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(rs,nr)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7750.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7755.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.54&0.24&173.5&0.54&0.48&20.7&
rs&0.94&0.77&32.9&1.29&0.93&85.5\\
&&&&&&&
bar&0.84&0.37&123.6&1.39&0.37&94.2\\
&&&&&&&
nr&0.12&0.09&28.5&0.14&0.12&83.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~7817}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~2492}}}\\
\multicolumn{7}{c}{SAB(rs,nd)bc }&
\multicolumn{7}{|c}{SAB(${\underline{\rm r}}$s)a/d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC7817.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC002492.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.66&0.26&50.8&0.86&0.63&71.7&
${\underline{\rm r}}$s&0.75&0.67&168.7&0.97&0.75&88.4\\
&&&&&&&
bar&0.37&0.17&171.5&0.38&0.24&13.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~3853}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~6228}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(${\underline{\rm r}}$s)cd }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC003853.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC006228.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&3.93&3.03&100.8&4.12&3.87&117.8&
r${\underline{\rm s}}$&1.06&0.31&65.9&1.14&0.75&149.4\\
${\underline{\rm r}}$s&1.55&1.12&78.9&1.76&1.32&123.5&
&&&&&&\\
bar&0.39&0.19&38.1&0.51&0.19&104.6&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~6626}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~11248}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(rs)cd }&
\multicolumn{7}{|c}{SB(rs)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC006626.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC011248.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.88&1.67&47.7&2.02&1.72&115.0&
rs&1.00&0.39&123.6&1.00&0.87&174.5\\
rs&0.92&0.75&40.4&0.99&0.77&116.4&
&&&&&&\\
bar&0.91&0.46&20.6&1.00&0.47&105.9&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf PGC~12633}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~12664}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(rs)ab }&
\multicolumn{7}{|c}{SA${\underline{\rm B}}$(r${\underline{\rm s}}$)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC012633.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC012664.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.66&0.56&99.0&0.66&0.57&42.3&
r${\underline{\rm s}}$&0.72&0.57&130.3&1.02&0.67&102.2\\
bar&0.63&0.31&99.4&0.63&0.31&39.7&
bar&0.17&0.07&88.1&0.28&0.08&101.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~12981}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~13684}}}\\
\multicolumn{7}{c}{SAB(s,nr?)m pec }&
\multicolumn{7}{|c}{SAB(r${\underline{\rm s}}$)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC012981.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC013684.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
bar&0.56&0.28&91.2&0.57&0.36&166.4&
r${\underline{\rm s}}$&0.59&0.26&167.0&0.59&0.48&2.2\\
nr&0.24&0.13&95.3&0.24&0.17&172.0&
bar&0.18&0.12&112.7&0.31&0.13&103.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~13716}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~14037}}}\\
\multicolumn{7}{c}{SA(r${\underline{\rm s}}$)c sp }&
\multicolumn{7}{|c}{SB(rs)c: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC013716.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC014037.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.48&0.12&138.7&0.48&0.29&4.9&
rs&0.40&0.25&129.1&0.56&0.39&102.8\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf PGC~32091}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~36274}}}\\
\multicolumn{7}{c}{S${\underline{\rm A}}$B(r${\underline{\rm s}}$)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SAB(s)m /RG }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC032091.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC036274.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.67&0.54&50.9&0.68&0.59&21.5&
R$^{\prime}$&1.09&0.67&57.4&1.17&0.91&41.1\\
bar&0.42&0.22&54.3&0.42&0.25&18.6&
bar&0.30&0.19&75.2&0.36&0.23&59.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~36551}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~36643}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SA(s)d }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(s)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC036551.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC036643.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.29&0.42&73.4&1.31&1.05&19.2&
R$^{\prime}$&1.58&0.52&139.1&1.93&1.44&60.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~38250}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~44735}}}\\
\multicolumn{7}{c}{SAB(rs)m: }&
\multicolumn{7}{|c}{SAB(rs)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC038250.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC044735.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.43&0.38&126.1&0.49&0.42&78.6&
rs&0.53&0.32&82.6&0.73&0.45&113.3\\
bar&0.38&0.19&65.0&0.43&0.21&125.1&
bar&0.25&0.17&56.1&0.44&0.19&102.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf PGC~44952}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~47721}}}\\
\multicolumn{7}{c}{SA(r)d: }&
\multicolumn{7}{|c}{SA(${\underline{\rm r}}$s,r$_{2}$,r$_{3}$)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC044952.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC047721.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.52&0.33&0.0&0.62&0.48&61.9&
${\underline{\rm r}}$s&1.47&0.74&117.5&1.49&1.27&162.7\\
&&&&&&&
r&1.12&0.48&117.5&1.12&0.82&169.2\\
&&&&&&&
r&0.70&0.34&116.4&0.71&0.58&161.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~48179}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~53093}}}\\
\multicolumn{7}{c}{SB(r${\underline{\rm s}}$)cd }&
\multicolumn{7}{|c}{(R$^{\prime}$R$^{\prime}$)SB(${\underline{\rm r}}$s)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC048179.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC053093.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&1.13&1.01&20.6&1.19&1.03&115.7&
R$^{\prime}$&1.03&0.59&100.8&1.05&1.00&135.8\\
bar&0.88&0.30&0.2&0.94&0.31&109.5&
R$^{\prime}$&0.66&0.42&95.7&0.75&0.64&115.5\\
&&&&&&&
${\underline{\rm r}}$s&0.31&0.17&98.1&0.32&0.29&140.2\\
&&&&&&&
bar&0.17&0.08&58.3&0.25&0.10&113.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~53415}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~54944}}}\\
\multicolumn{7}{c}{(R)Sph/SA(rs)a }&
\multicolumn{7}{|c}{SB(${\underline{\rm r}}$s)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC053415.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC054944.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R&1.86&0.63&47.4&1.86&1.19&0.4&
bar&0.60&0.15&35.3&0.62&0.21&22.0\\
rs&0.29&0.08&50.1&0.29&0.16&7.1&
${\underline{\rm r}}$s&0.58&0.30&10.8&0.59&0.42&157.9\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf PGC~66242}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~313}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)d }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$)SB$_{\rm a}$(s)b /Sph }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC066242.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC00313.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.45&0.66&39.1&1.49&1.40&140.3&
R$_{1}^{\prime}$&0.38&0.15&14.9&0.38&0.24&0.1\\
&&&&&&&
bar&0.14&0.04&102.6&0.23&0.04&88.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~1551}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~1862}}}\\
\multicolumn{7}{c}{SB(rs)cd }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(s)b: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC01551.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC01862.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.65&0.55&170.7&0.73&0.57&69.0&
R$^{\prime}$&0.79&0.65&2.4&0.85&0.74&121.5\\
bar&0.57&0.19&81.2&0.62&0.21&132.7&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~4151}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~4306}}}\\
\multicolumn{7}{c}{SA(rl)c }&
\multicolumn{7}{|c}{SA(r)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04151.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04306.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rl&0.12&0.10&36.0&0.13&0.10&73.3&
r&0.21&0.06&140.2&0.21&0.10&5.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf UGC~4549}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~4551}}}\\
\multicolumn{7}{c}{SA(r)c }&
\multicolumn{7}{|c}{SB(r)0$^{+}$ sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04549.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04551.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.18&0.16&84.2&0.22&0.16&83.4&
r&1.00&0.26&113.4&1.01&0.68&6.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~4559}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~4621}}}\\
\multicolumn{7}{c}{SA(r)0/a }&
\multicolumn{7}{|c}{SB(${\underline{\rm r}}$s)ab }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04559.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04621.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&0.51&0.08&51.1&0.51&0.28&2.1&
${\underline{\rm r}}$s&0.56&0.33&132.1&0.56&0.55&142.6\\
&&&&&&&
bar&0.48&0.19&150.6&0.53&0.28&35.2\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~4623}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~4714}}}\\
\multicolumn{7}{c}{SA(rs)bc }&
\multicolumn{7}{|c}{S${\underline{\rm A}}$B(rs)m }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04623.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04714.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.31&0.14&56.6&0.51&0.31&92.9&
rs&0.27&0.22&100.3&0.27&0.27&90.0\\
&&&&&&&
bar&0.21&0.11&59.4&0.24&0.12&129.5\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf UGC~4824}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~4867}}}\\
\multicolumn{7}{c}{SB(rs)d }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04824.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04867.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.89&0.28&95.4&1.04&0.84&116.8&
r${\underline{\rm s}}$&0.41&0.25&94.8&0.42&0.40&35.6\\
&&&&&&&
bar&0.14&0.07&179.4&0.23&0.07&88.6\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~4922}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~4982}}}\\
\multicolumn{7}{c}{SAB(rs)cd }&
\multicolumn{7}{|c}{SA(r)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04922.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC04982.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.78&0.45&52.6&1.01&0.76&103.4&
r&0.25&0.12&176.4&0.31&0.24&113.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~5228}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~5354}}}\\
\multicolumn{7}{c}{(R$_{2}^{\prime}$)SB(s)cd }&
\multicolumn{7}{|c}{(R:)SAB(s)dm }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05228.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05354.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$_{2}^{\prime}$&1.81&0.38&123.8&1.81&1.25&0.0&
R&0.98&0.63&79.0&1.11&0.97&80.7\\
&&&&&&&
bar&0.56&0.23&71.5&0.56&0.41&165.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf UGC~5393}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~5446}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)m }&
\multicolumn{7}{|c}{SAB(rs)dm sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05393.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05446.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.94&0.63&122.0&1.24&0.93&83.9&
rs&0.28&0.13&47.8&0.56&0.28&93.6\\
bar&0.19&0.08&145.7&0.25&0.11&56.0&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~5633}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~5646}}}\\
\multicolumn{7}{c}{SB(rs)dm }&
\multicolumn{7}{|c}{SA:(rs:)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05633.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05646.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.01&0.69&160.3&1.17&0.94&116.1&
rs&0.49&0.14&169.3&0.53&0.43&40.0\\
bar&0.79&0.15&162.9&0.82&0.23&161.6&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~5676}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~5707}}}\\
\multicolumn{7}{c}{SA${\underline{\rm B}}$(s)m:/RG? }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05676.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05707.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RG&1.09&0.50&22.3&1.12&0.89&24.7&
r${\underline{\rm s}}$&0.32&0.21&59.8&0.39&0.22&77.8\\
bar&0.16&0.10&88.6&0.29&0.10&83.2&
bar&0.18&0.07&64.9&0.21&0.07&79.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf UGC~5814}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~5841}}}\\
\multicolumn{7}{c}{(RL)SB0/a (shells?) pec }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(r${\underline{\rm s}}$:)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05814.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC05841.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&0.52&0.41&105.2&0.74&0.48&104.1&
R$^{\prime}$&0.76&0.45&127.0&0.82&0.74&116.8\\
&&&&&&&
bar&0.43&0.14&136.7&0.43&0.25&11.6\\
&&&&&&&
r${\underline{\rm s}}$&0.38&0.21&136.1&0.40&0.35&33.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~6023}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~6162}}}\\
\multicolumn{7}{c}{SAB(${\underline{\rm r}}$s)c }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(s)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC06023.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC06162.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
${\underline{\rm r}}$s&0.43&0.22&48.0&0.45&0.42&129.8&
R$^{\prime}$&1.67&0.94&90.6&1.74&1.54&38.9\\
bar&0.38&0.12&47.7&0.38&0.23&173.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~6169}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~6309}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB$_{\rm a}$(s)b: sp }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC06169.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC06309.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&0.59&0.10&178.4&0.61&0.34&162.6&
r${\underline{\rm s}}$&0.69&0.50&104.2&0.72&0.57&144.0\\
&&&&&&&
bar&0.61&0.13&139.7&0.61&0.15&16.7\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf UGC~6335}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~6517}}}\\
\multicolumn{7}{c}{SAB(rs)c }&
\multicolumn{7}{|c}{SA(r)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC06335.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC06517.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.20&0.15&160.4&0.24&0.15&91.1&
r&0.32&0.18&21.4&0.35&0.28&131.3\\
bar&0.14&0.09&51.4&0.15&0.11&154.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~6983}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~7184}}}\\
\multicolumn{7}{c}{SB(r)s)dm pec }&
\multicolumn{7}{|c}{SB(rs)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC06983.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC07184.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r&1.04&0.99&113.3&1.51&1.03&86.9&
rs&0.64&0.28&147.5&0.65&0.54&25.0\\
bar&0.94&0.28&89.0&0.94&0.42&3.5&
bar&0.47&0.12&163.5&0.57&0.21&41.5\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~7239}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~7848}}}\\
\multicolumn{7}{c}{(R$^{\prime}$)SB(s)m }&
\multicolumn{7}{|c}{SAB$_{\rm a}$(s,x$_{1}$r)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC07239.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC07848.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.24&1.10&11.1&1.54&1.11&86.1&
x$_{1}$r&0.30&0.14&75.3&0.40&0.24&59.9\\
bar&0.36&0.19&21.3&0.45&0.19&89.2&
&&&&&&\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf UGC~8155}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~8909}}}\\
\multicolumn{7}{c}{SA(rs,l)a }&
\multicolumn{7}{|c}{SAB(r${\underline{\rm s}}$)c: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC08155.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC08909.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.24&0.90&12.8&1.24&1.13&172.4&
r${\underline{\rm s}}$&0.28&0.19&68.5&0.28&0.23&21.2\\
&&&&&&&
bar&0.17&0.11&131.3&0.20&0.11&79.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~8995}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~9215}}}\\
\multicolumn{7}{c}{(R$^{\prime}$:)SA(s)cd: }&
\multicolumn{7}{|c}{(R$^{\prime}$)SB(r${\underline{\rm s}}$)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC08995.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09215.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$&1.44&0.62&6.7&1.51&1.29&38.0&
R$^{\prime}$&1.60&0.70&160.5&1.60&1.56&168.4\\
&&&&&&&
r${\underline{\rm s}}$&0.94&0.58&157.1&1.31&0.93&95.4\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~9245}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~9291}}}\\
\multicolumn{7}{c}{SB(rs)dm }&
\multicolumn{7}{|c}{SAB(rs)bc }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09245.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09291.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.21&0.64&173.2&1.21&0.88&171.7&
rs&0.50&0.32&110.9&0.59&0.49&71.3\\
bar&0.26&0.03&9.3&0.26&0.04&16.6&
bar&0.23&0.10&84.7&0.27&0.16&136.4\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf UGC~9356}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~9364}}}\\
\multicolumn{7}{c}{(R$^{\prime}$L)SAB(rs)bc: }&
\multicolumn{7}{|c}{(R$^{\prime}$)SA(s)cd }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09356.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09364.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
R$^{\prime}$L&1.07&0.45&107.0&1.08&0.86&13.6&
R$^{\prime}$&0.91&0.40&17.8&0.92&0.81&164.8\\
rs&0.59&0.27&99.2&0.61&0.51&152.9&
&&&&&&\\
bar&0.24&0.10&60.8&0.37&0.12&113.4&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~9389}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~9569}}}\\
\multicolumn{7}{c}{SB(rs)dm }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)c }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09389.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09569.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.24&0.34&47.1&1.27&1.21&136.5&
r${\underline{\rm s}}$&0.69&0.46&168.1&0.80&0.51&60.3\\
&&&&&&&
bar&0.43&0.17&168.8&0.50&0.19&53.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~9746}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~9858}}}\\
\multicolumn{7}{c}{SB(rs)cd sp }&
\multicolumn{7}{|c}{SA(rs)b }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09746.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC09858.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.97&0.19&137.8&0.97&0.71&179.3&
rs&0.46&0.13&67.5&0.62&0.36&123.1\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf UGC~10054}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~10791}}}\\
\multicolumn{7}{c}{SB(rs)d }&
\multicolumn{7}{|c}{SB(rs)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC10054.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC10791.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&1.13&0.56&145.1&1.15&1.04&27.7&
rs&0.70&0.53&111.4&0.86&0.68&75.5\\
bar&0.60&0.10&154.0&0.64&0.18&23.4&
bar&0.29&0.12&155.9&0.42&0.13&70.0\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf UGC~10854}}}&
\multicolumn{7}{|c}{{\large{\bf UGC~12151}}}\\
\multicolumn{7}{c}{SAB(r${\underline{\rm s}}$)m }&
\multicolumn{7}{|c}{SB(r${\underline{\rm s}}$)d }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/UGC10854.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/UGC12151.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
r${\underline{\rm s}}$&0.44&0.24&79.0&0.60&0.41&110.3&
r${\underline{\rm s}}$&0.60&0.47&7.5&0.78&0.59&81.3\\
&&&&&&&
bar&0.26&0.07&173.8&0.26&0.12&173.3\\
\hline
\\
\end{longtable}
\clearpage
\subsection{Atlas of galaxies not in the S$^4$G sample that host rings}
\begin{longtable}{c c c c c c c | c c c c c c c}
\multicolumn{7}{c}{{\large{\bf IC~3062}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~2856}}}\\
\multicolumn{7}{c}{SA(rs)bc }&
\multicolumn{7}{|c}{SAB(r)a: }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/IC3062.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2856.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.27&0.21&149.9&0.30&0.23&119.1&
r&0.37&0.16&144.6&0.43&0.28&47.1\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~2950}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4175}}}\\
\multicolumn{7}{c}{(RL)SA${\underline{\rm B}}$$_{\rm a}$(r${\underline{\rm l}}$,bl)0$^{+}$ }&
\multicolumn{7}{|c}{SA(r,PR?)0/a sp }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC2950.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4175.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
RL&1.99&1.50&115.9&2.25&1.96&104.8&
r&0.41&0.11&130.4&0.41&0.32&176.0\\
r${\underline{\rm l}}$&0.97&0.68&122.2&1.00&0.97&93.9&
PRG&0.29&0.03&38.7&$-$&$-$&$-$\\
bar&0.80&0.47&155.7&0.98&0.57&56.5&
&&&&&&\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf NGC~4277}}}&
\multicolumn{7}{|c}{{\large{\bf NGC~4288A}}}\\
\multicolumn{7}{c}{SAB(rs)0$^{+}$ }&
\multicolumn{7}{|c}{(L)S${\underline{\rm A}}$B(rl)0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4277.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4288A.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.57&0.43&117.5&0.59&0.57&87.9&
rl&0.25&0.25&40.7&0.26&0.25&89.7\\
bar&0.41&0.25&169.7&0.51&0.27&67.0&
bar&0.23&0.17&161.2&0.24&0.17&115.5\\
\hline
\\
\\
\pagebreak
\multicolumn{7}{c}{{\large{\bf NGC~4342}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~43690}}}\\
\multicolumn{7}{c}{S0$^{-}$ sp + vF PR? }&
\multicolumn{7}{|c}{(R$_{1}^{\prime}$)SAB$_{\rm a}$(ls)a }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/NGC4342.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC043690.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
PRG&0.40&0.04&80.7&$-$&$-$&$-$&
R$_{1}^{\prime}$&0.80&0.40&108.9&0.81&0.60&169.2\\
&&&&&&&
bar&0.16&0.13&18.8&0.25&0.13&88.7\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~50803}}}&
\multicolumn{7}{|c}{{\large{\bf PGC~52269}}}\\
\multicolumn{7}{c}{SB(rs)a }&
\multicolumn{7}{|c}{(R)SB0$^{+}$ }\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC050803.eps}}&
\multicolumn{7}{|c}{\includegraphics[width=0.48\textwidth]{atlas/PGC052269.eps}}\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ & Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$\\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)\\
\hline
rs&0.31&0.19&94.4&0.32&0.24&145.7&
R&0.35&0.33&130.1&0.36&0.35&71.2\\
bar&0.30&0.10&114.2&0.30&0.14&7.2&
bar&0.17&0.12&165.4&0.18&0.13&50.3\\
\hline
\\
\multicolumn{7}{c}{{\large{\bf PGC~59663}}}&
\\
\multicolumn{7}{c}{(R$^{\prime}$)Sa sp }&
\\
\multicolumn{7}{c}{\includegraphics[width=0.48\textwidth]{atlas/PGC059663.eps}}&
\\
\hline\hline
Feature & $D_{\rm r,b}$ & $d_{\rm r,b}$ & ${\rm PA_{r,b}}$ & $D_{\rm r,b,0}$ & $d_{\rm r,b,0}$ & ${\theta_{\rm r,b}}$ \\
&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&($\arcmin$) & ($\arcmin$) & ($^{\rm o}$)&\\
\hline
R$^{\prime}$&0.37&0.10&87.0&0.41&0.29&141.9&
\\
\hline
\pagebreak
\end{longtable}


==> fSA.tex <==
$47\pm3\%$


==> fSAB_.tex <==
$68\pm7\%$


==> nKOR079.tex <==
          32


==> nKOR79.tex <==
          97


==> nRC3.tex <==
        2282


==> ndeVA.tex <==
         303


==> nfpringsearlyS0.tex <==
$28\pm8\%


==> nfratioe.tex <==
$28\%$


==> nfratiol.tex <==
$47\%$


==> nmisinterm.tex <==
          20


==> nnoinRC3.tex <==
          66


==> nnotype.tex <==
          37


==> nnotyperinged.tex <==
none


==> nstage.tex <==
        2265


==> tinnerCSRG.tex <==
\begin{table*}
\caption{Comparison of the inner (pseudo)ring properties in the S$^4$G and the CSRG}
\label{tinnerCSRG}
\centering
\begin{tabular}{c c |c c c c c c}
\hline\hline
& &\multicolumn{6}{c}{CSRG}\\
& &s&r${\underline{\rm s}}$&rs&${\underline{\rm r}}$s&r&l\\
\hline
\multirow{8}{*}{S$^4$G}
&s
&9 (8\%)
&5 (4\%)
&15 (13\%)
&1 (1\%)
&8 (7\%)
&0 (0\%)\\
&r${\underline{\rm s}}$
&3 (3\%)
&2 (2\%)
&5 (4\%)
&1 (1\%)
&1 (1\%)
&0 (0\%)\\
&rs
&1 (1\%)
&3 (3\%)
&10 (8\%)
&3 (3\%)
&15 (13\%)
&0 (0\%)\\
&${\underline{\rm r}}$s
&0 (0\%)
&0 (0\%)
&2 (2\%)
&1 (1\%)
&5 (4\%)
&0 (0\%)\\
&r
&0 (0\%)
&0 (0\%)
&2 (2\%)
&1 (1\%)
&16 (13\%)
&0 (0\%)\\
&Multiple
&0 (0\%)
&0 (0\%)
&1 (1\%)
&1 (1\%)
&1 (1\%)
&0 (0\%)\\
&l
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&3 (3\%)
&1 (1\%)\\
&No variety
&2 (2\%)
&0 (0\%)
&1 (1\%)
&1 (1\%)
&0 (0\%)
&0 (0\%)\\
\hline
\end{tabular}
\end{table*}


==> tinnerKOR079.tex <==
\begin{table}
\caption{Comparison of the inner (pseudo)ring properties in the S$^4$G and the \citet{KOR79} samples}
\label{tinnerKOR79}
\centering
\begin{tabular}{c c |c c c c}
\hline\hline
& &\multicolumn{4}{c}{\citet{KOR79}}\\
& &None&r$^{\prime}$&r&l\\
\hline
\multirow{8}{*}{S$^4$G}
&s
&20 (21\%)
&0 (0\%)
&1 (1\%)
&1 (1\%)\\
&r${\underline{\rm s}}$
&4 (4\%)
&0 (0\%)
&2 (2\%)
&0 (0\%)\\
&rs
&8 (8\%)
&3 (3\%)
&8 (8\%)
&2 (2\%)\\
&${\underline{\rm r}}$s
&1 (1\%)
&1 (1\%)
&8 (8\%)
&1 (1\%)\\
&r
&2 (2\%)
&0 (0\%)
&14 (14\%)
&5 (5\%)\\
&Multiple
&0 (0\%)
&0 (0\%)
&1 (1\%)
&0 (0\%)\\
&l
&2 (2\%)
&0 (0\%)
&0 (0\%)
&1 (1\%)\\
&No variety
&9 (9\%)
&0 (0\%)
&0 (0\%)
&3 (3\%)\\
\hline
\end{tabular}
\end{table}


==> tinnerNIRS0S.tex <==
\begin{table*}
\caption{Comparison of the inner (pseudo)ring properties in the S$^4$G and NIRS0S}
\label{tinnernirs0s}
\centering
\begin{tabular}{c c |c c c c c c c c}
\hline\hline
& &\multicolumn{8}{c}{NIRS0S}\\
& &s&r${\underline{\rm s}}$&rs&${\underline{\rm r}}$s&r&Multiple &l & No variety\\
\hline
\multirow{8}{*}{S$^4$G}
&s
&7 (8\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&1 (1\%)
&0 (0\%)
&0 (0\%)
&4 (4\%)\\
&r${\underline{\rm s}}$
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)\\
&rs
&1 (1\%)
&0 (0\%)
&7 (8\%)
&0 (0\%)
&2 (2\%)
&0 (0\%)
&1 (1\%)
&0 (0\%)\\
&${\underline{\rm r}}$s
&1 (1\%)
&0 (0\%)
&3 (3\%)
&5 (5\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)\\
&r
&1 (1\%)
&1 (1\%)
&3 (3\%)
&2 (2\%)
&18 (19\%)
&2 (2\%)
&2 (2\%)
&2 (2\%)\\
&Multiple
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&1 (1\%)
&1 (1\%)
&0 (0\%)
&0 (0\%)\\
&l
&1 (1\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&1 (1\%)
&0 (0\%)
&6 (6\%)
&2 (2\%)\\
&No variety
&1 (1\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&2 (2\%)
&15 (16\%)\\
\hline
\end{tabular}
\end{table*}


==> tinnerRC3.tex <==
\begin{table*}
\caption{Comparison of the inner (pseudo)ring properties in the S$^4$G and the RC3 sample}
\label{tinnerRC3}
\centering
\begin{tabular}{c c |c c c c}
\hline\hline
& &\multicolumn{4}{c}{RC3}\\
& &s&r$^{\prime}$&r&No variety\\
\hline
\multirow{8}{*}{S$^4$G}
&s
&399 (17\%)
&137 (6\%)
&22 (1\%)
&392 (17\%)\\
&r${\underline{\rm s}}$
&35 (2\%)
&36 (2\%)
&5 (0\%)
&20 (1\%)\\
&rs
&71 (3\%)
&86 (4\%)
&23 (1\%)
&63 (3\%)\\
&${\underline{\rm r}}$s
&12 (1\%)
&21 (1\%)
&29 (1\%)
&10 (0\%)\\
&r
&29 (1\%)
&28 (1\%)
&60 (3\%)
&44 (2\%)\\
&Multiple
&3 (0\%)
&7 (0\%)
&4 (0\%)
&0 (0\%)\\
&l
&20 (1\%)
&6 (0\%)
&10 (0\%)
&29 (1\%)\\
&No variety
&124 (5\%)
&10 (0\%)
&11 (0\%)
&536 (23\%)\\
\hline
\end{tabular}
\end{table*}


==> tinnerVAU80.tex <==
\begin{table}
\caption{Comparison of the inner (pseudo)ring properties in the S$^4$G and the \citet{VAU80} sample}
\label{tinnerVAU80}
\centering
\begin{tabular}{c c |c c c c}
\hline\hline
& &\multicolumn{4}{c}{\citet{VAU80}}\\
& &None&r$^{\prime}$&r&Multiple\\
\hline
\multirow{8}{*}{S$^4$G}
&s
&6 (2\%)
&43 (14\%)
&13 (4\%)
&0 (0\%)\\
&r${\underline{\rm s}}$
&5 (2\%)
&24 (8\%)
&2 (1\%)
&0 (0\%)\\
&rs
&15 (5\%)
&37 (12\%)
&25 (8\%)
&0 (0\%)\\
&${\underline{\rm r}}$s
&3 (1\%)
&11 (4\%)
&21 (7\%)
&0 (0\%)\\
&r
&1 (0\%)
&13 (4\%)
&57 (19\%)
&0 (0\%)\\
&Multiple
&0 (0\%)
&3 (1\%)
&3 (1\%)
&0 (0\%)\\
&l
&5 (2\%)
&4 (1\%)
&2 (1\%)
&0 (0\%)\\
&No variety
&1 (0\%)
&3 (1\%)
&5 (2\%)
&1 (0\%)\\
\hline
\end{tabular}
\end{table}


==> tinnerdeVA.tex <==
\begin{table*}
\caption{Comparison of the inner (pseudo)ring properties in the S$^4$G and the \citet{BU07}}
\label{tinnerdeVA}
\centering
\begin{tabular}{c c |c c c c c c c}
\hline\hline
& &\multicolumn{6}{c}{\citet{BU07}}\\
& &s&r${\underline{\rm s}}$&rs&${\underline{\rm r}}$s&r&l&No variety\\
\hline
\multirow{8}{*}{S$^4$G}
&s
&64 (21\%)
&1 (0\%)
&9 (3\%)
&0 (0\%)
&1 (0\%)
&0 (0\%)
&5 (2\%)\\
&r${\underline{\rm s}}$
&8 (3\%)
&7 (2\%)
&6 (2\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)\\
&rs
&16 (5\%)
&7 (2\%)
&26 (9\%)
&2 (1\%)
&5 (2\%)
&0 (0\%)
&1 (0\%)\\
&${\underline{\rm r}}$s
&3 (1\%)
&0 (0\%)
&5 (2\%)
&11 (4\%)
&3 (1\%)
&0 (0\%)
&0 (0\%)\\
&r
&2 (1\%)
&2 (1\%)
&4 (1\%)
&5 (2\%)
&32 (11\%)
&2 (1\%)
&6 (2\%)\\
&Multiple
&1 (0\%)
&1 (0\%)
&0 (0\%)
&1 (0\%)
&3 (1\%)
&0 (0\%)
&0 (0\%)\\
&l
&4 (1\%)
&0 (0\%)
&2 (1\%)
&0 (0\%)
&3 (1\%)
&2 (1\%)
&3 (1\%)\\
&No variety
&11 (4\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&39 (13\%)\\
\hline
\end{tabular}
\end{table*}


==> tnuclearNIRS0S.tex <==
\begin{table}
\caption{Comparison of the nuclear (pseudo)ring properties in the S$^4$G and NIRS0S}
\label{tnuclearnirs0s}
\centering
\begin{tabular}{c c |c c c c}
\hline\hline
& &\multicolumn{4}{c}{NIRS0S}\\
& &none&nr$^{\prime}$&nr&nl\\
\hline
\multirow{4}{*}{S$^4$G}
&None
&63 (68\%)
&0 (0\%)
&2 (2\%)
&6 (6\%)\\
&nr$^{\prime}$
&0 (0\%)
&0 (0\%)
&0 (0\%)
&1 (1\%)\\
&nr
&0 (0\%)
&1 (1\%)
&8 (9\%)
&0 (0\%)\\
&nl
&2 (2\%)
&0 (0\%)
&3 (3\%)
&7 (8\%)\\
\hline
\end{tabular}
\end{table}


==> touterCSRG.tex <==
\begin{table*}
\caption{Comparison of the outer (pseudo)ring properties in the S$^4$G and the CSRG}
\label{touterCSRG}
\centering
\begin{tabular}{c c |c c c c c}
\hline\hline
& &\multicolumn{5}{c}{CSRG}\\
& &None&R$^{\prime}$&R&Multiple&L\\
\hline
\multirow{5}{*}{S$^4$G}
&None
&58 (48\%)
&7 (6\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)\\
&R$^{\prime}$
&10 (8\%)
&19 (16\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)\\
&R
&2 (2\%)
&4 (3\%)
&8 (7\%)
&3 (3\%)
&1 (1\%)\\
&Multiple
&2 (2\%)
&2 (2\%)
&0 (0\%)
&1 (1\%)
&0 (0\%)\\
&L
&1 (1\%)
&0 (0\%)
&0 (0\%)
&1 (1\%)
&1 (1\%)\\
\hline
\end{tabular}
\end{table*}


==> touterNIRS0S.tex <==
\begin{table*}
\caption{Comparison of the outer (pseudo)ring properties in the S$^4$G and NIRS0S}
\label{touternirs0s}
\centering
\begin{tabular}{c c |c c c c c}
\hline\hline
& &\multicolumn{5}{c}{NIRS0S}\\
& &None&R$^{\prime}$&R&Multiple&L\\
\hline
\multirow{5}{*}{S$^4$G}
&None
&31 (33\%)
&0 (0\%)
&0 (0\%)
&0 (0\%)
&2 (2\%)\\
&R$^{\prime}$
&2 (2\%)
&5 (5\%)
&1 (1\%)
&0 (0\%)
&0 (0\%)\\
&R
&5 (5\%)
&6 (6\%)
&16 (17\%)
&0 (0\%)
&1 (1\%)\\
&Multiple
&2 (2\%)
&0 (0\%)
&3 (3\%)
&1 (1\%)
&0 (0\%)\\
&L
&7 (8\%)
&1 (1\%)
&4 (4\%)
&0 (0\%)
&6 (6\%)\\
\hline
\end{tabular}
\end{table*}


==> touterRC3.tex <==
\begin{table}
\caption{Comparison of the outer (pseudo)ring properties in the S$^4$G and the RC3 sample}
\label{touterRC3}
\centering
\begin{tabular}{c c |c c c}
\hline\hline
& &\multicolumn{3}{c}{RC3}\\
& &None&R$^{\prime}$&R\\
\hline
\multirow{5}{*}{S$^4$G}
&None
&1921 (84\%)
&27 (1\%)
&12 (1\%)\\
&R$^{\prime}$
&138 (6\%)
&20 (1\%)
&11 (0\%)\\
&R
&54 (2\%)
&12 (1\%)
&23 (1\%)\\
&Multiple
&10 (0\%)
&0 (0\%)
&7 (0\%)\\
&L
&42 (2\%)
&3 (0\%)
&2 (0\%)\\
\hline
\end{tabular}
\end{table}


==> touterVAU80.tex <==
\begin{table}
\caption{Comparison of the outer (pseudo)ring properties in the S$^4$G and the \citet{VAU80} sample}
\label{touterVAU80}
\centering
\begin{tabular}{c c |c c c}
\hline\hline
& &\multicolumn{3}{c}{\citet{VAU80}}\\
& &None&R$^{\prime}$&R\\
\hline
\multirow{5}{*}{S$^4$G}
&None
&147 (49\%)
&24 (8\%)
&5 (2\%)\\
&R$^{\prime}$
&30 (10\%)
&25 (8\%)
&5 (2\%)\\
&R
&14 (5\%)
&16 (5\%)
&13 (4\%)\\
&Multiple
&2 (1\%)
&6 (2\%)
&4 (1\%)\\
&L
&11 (4\%)
&0 (0\%)
&1 (0\%)\\
\hline
\end{tabular}
\end{table}


==> touterdeVA.tex <==
\begin{table}
\caption{Comparison of the outer (pseudo)ring properties in the S$^4$G and the \citet{BU07}}
\label{touterdeVA}
\centering
\begin{tabular}{c c |c c c c}
\hline\hline
& &\multicolumn{4}{c}{\citet{BU07}}\\
& &None&R$^{\prime}$&R&Multiple\\
\hline
\multirow{5}{*}{S$^4$G}
&None
&192 (63\%)
&4 (1\%)
&2 (1\%)
&0 (0\%)\\
&R$^{\prime}$
&19 (6\%)
&25 (8\%)
&3 (1\%)
&2 (1\%)\\
&R
&6 (2\%)
&11 (4\%)
&17 (6\%)
&2 (1\%)\\
&Multiple
&2 (1\%)
&4 (1\%)
&1 (0\%)
&1 (0\%)\\
&L
&10 (3\%)
&0 (0\%)
&1 (0\%)
&1 (0\%)\\
\hline
\end{tabular}
\end{table}

